Henge: Intent-driven Multi-Tenant Stream Processing

We present Henge, a system to support intent-based multi-tenancy in modern stream processing applications. Henge supports multi-tenancy as a first-class citizen: everyone inside an organization can now submit their stream processing jobs to a single, shared, consolidated cluster. Additionally, Henge allows each tenant (job) to specify its own intents (i.e., requirements) as a Service Level Objective (SLO) that captures latency and/or throughput. In a multi-tenant cluster, the Henge scheduler adapts continually to meet jobs' SLOs in spite of limited cluster resources, and under dynamic input workloads. SLOs are soft and are based on utility functions. Henge continually tracks SLO satisfaction, and when jobs miss their SLOs, it wisely navigates the state space to perform resource allocations in real time, maximizing total system utility achieved by all jobs in the system. Henge is integrated in Apache Storm and we present experimental results using both production topologies and real datasets.

==> henge-arxiv 2/preamble.tex <==
\usepackage{epsfig,endnotes,algorithm,verbatim,algpseudocode}
\usepackage{amsmath}
\usepackage{balance}
\usepackage{flushend}
\usepackage{multirow}
\usepackage{color}
\usepackage{wrapfig}
\usepackage{graphicx}
\usepackage[font=small,labelfont=bf]{caption}
\usepackage{url}
\usepackage{subcaption}
\usepackage{booktabs}
\usepackage{mwe}
\usepackage{hyperref}
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\usepackage{times}
\usepackage{datetime}
\usepackage{url}

\usepackage[numbers]{natbib}


\usepackage{etoolbox}
%------------------------------------------


 \newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
    \end{list}  }


==> henge-arxiv 2/text/00-abstract.tex <==
\begin{abstract}
We present Henge,  a system to support intent-based multi-tenancy in modern stream processing applications.  Henge supports multi-tenancy as a first-class citizen: everyone inside an organization can now submit their stream processing jobs to a single, shared, consolidated cluster. Additionally, Henge allows each tenant (job) to specify its own intents (i.e., requirements) as a Service Level Objective (SLO) that captures latency and/or throughput. In a multi-tenant cluster, the Henge  scheduler adapts continually to meet jobs' SLOs in spite of limited cluster resources, and  under dynamic input workloads.  SLOs are soft and are based on utility functions. Henge continually tracks SLO satisfaction, and when jobs miss their SLOs, it wisely navigates the state space to perform resource allocations in real time,  maximizing total system utility achieved by all jobs in the system. Henge is integrated in Apache Storm and we present experimental results using both production topologies and real datasets. 
\end{abstract}
%self-adapts
% stream processing
%ally varying
% Each tenant as SLOs (Service Level Objectives): each tenant (i.e., a job, e.g.,
% topology in Apache Storm) specifies either a latency SLO or a throughput SLO. ,
% or a combination thereof.


==> henge-arxiv 2/text/01-introduction.tex <==
\section{Introduction}
\label{introduction}

% \ig{Don't touch, though you can comment}

Modern stream processing systems  process continuously-arriving data streams in real time, ranging from Web data to social network streams. For instance, several companies use Apache Storm~\cite{storm_web} (e.g., Weather Channel, Alibaba, Baidu, WebMD, etc.),  Twitter uses Heron~\cite{heron}, LinkedIn relies on Samza~\cite{samza} and others use Apache Flink~\cite{flink}. These systems provide high-throughput and low-latency processing of streaming data from advertisement pipelines  (Yahoo! Inc. uses Storm for this), social network posts (LinkedIn, Twitter), geospatial data (Twitter), etc.

While stream processing systems for clusters have been around for decades~\cite{borealis, spade}, modern stream processing systems have scant support for {\it intent-based multi-tenancy}. We tease apart these two terms. First,  multi-tenancy allows multiple jobs to share a single consolidated cluster.  This capability is lacking in stream processing systems today--as a result,  many companies (e.g., Yahoo!) over-provision the stream processing cluster   and then physically apportion it among tenants (often based  on team priority). Besides higher cost, this entails manual administration  of multiple clusters and caps on allocation by the sysadmin, and manual monitoring of job behavior by each deployer. %(e.g., this is the case inside Yahoo!)

Multi-tenancy is attractive as it reduces acquisition costs and allows sysadmins to only manage a single consolidated cluster. Thus, this approach reduces capital and operational expenses (Capex \& Opex), lowers  total cost of ownership (TCO),  increases resource utilization, and allows jobs to elastically scale based on needs. Multi-tenancy has been explored for  areas such as key-value stores \cite{shue2012performance}, storage systems~\cite{wang2012cake}, batch processing \cite{yarn}, and others~\cite{mace2015retro}, yet it remains a vital need in modern stream processing systems. %\fkc{I propose switching the order of the last paragraph with a section from the second-last, starting from ``This capability is lacking ...''} %The notion of m

Second, we believe the deployer of each job should be able to clearly specify their performance expectations as an intent to the system, and it is the underlying engine's responsibility to meet this intent. This alleviates the developer's burden of monitoring and adjusting their job. Modern open-source stream processing systems like Storm~\cite{storm-multitenant-scheduler}  are very primitive and do not admit intents of any kind. %Analogous to recent developments in the area of intent-based networking~\cite{lerner17}, our work brings intent-based notions to distributed systems scheduling (focusing on stream processing). 


% \fkc{in a multi-tenant environment}
%\fkc{Then, Henge is responsible for translating these intents to  resource configurations that allow the jobs to satisfy their SLOs.}

Our approach is to allow each job in a multi-tenant environment to specify its intent as a Service Level Objective (SLO). The   metrics  in an SLO should be {\it user-facing}, i.e., understandable and settable by lay users such as a deployer who is not intimately familiar with the innards of the system. For instance, SLO metrics can capture latency and throughput expectations. SLOs do not include internal metrics like queue lengths or CPU utilization which can vary depending on the software, cluster, and job mix\footnote{However, these latter metrics can be monitored and used internally by the scheduler for self-adaptation.}. We believe lay users should not have to grapple with such complex metrics. 




While there are myriad ways to specify SLOs (including potentially declarative languages paralleling SQL), our paper is best seen as one contributing {\it mechanisms} that are pivotal in order to build a truly intent-based distributed system for stream processing. In spite of their simplicity, our latency and throughput SLOs are immediately useful. Time-sensitive jobs (e.g., those related to an ongoing ad campaign) are latency-sensitive and can specify latency SLOs, while longer running jobs (e.g., sentiment analysis of trending topics) typically have throughput SLOs. %Support for a multi-tenant cluster with SLOs eliminates the need for over-provisioning. Instead of the de facto style today of statically partitioning a cluster for  jobs, consolidation makes the cluster shared, more effective, and cost-efficient. 


%Table~\ref{henge-comparison} compares Henge with existing schedulers that handle multi-tenancy. 


\begin{table}[t]
% \vspace{-0.4em}
\centering
\resizebox{0.50\textwidth}{!}{%
\begin{tabular}{l l l l l}
\toprule%\hline
Schedulers & Job Type & Adaptive & Reservation-Based & SLOs  \\ \hline
Mesos~\cite{mesos} & General & \xmark & \cmark (CPU, Mem, Disk, Ports) & \xmark \\ \hline
YARN~\cite{yarn} & General & \xmark & \cmark (CPU, Mem, Disk) & \xmark \\ \hline
%Henge & Stream & \cmark & \xmark \ (User-facing SLOs) & \cmark \\ \hline
%Rayon~\cite{curino2014reservation} & Batch & \cmark  & \cmark (Resources across time) & \cmark \\ %\hline
Rayon~\cite{curino2014reservation} & Batch & \cmark  & \cmark (Resources across time) & \cmark \\ \hline
{\bf Henge} & {\bf Stream} & \cmark & \xmark \ {\bf (User-facing SLOs)} & \cmark \\ %\hline
\bottomrule
\end{tabular}%
}
 \vspace{-0.3cm}
\caption{\bf Henge vs. Existing Schedulers.}
\vspace{-0.5cm}
\label{henge-comparison}

\end{table}



%We present the {Henge} system, an intent-driven multi-tenant scheduler aimed at clusters containing stream processing applications. 

As Table~\ref{henge-comparison} shows, most existing schedulers use reservation-based approaches to specify intents: besides not being user-facing, these are very hard to estimate even for a job with a static workload~\cite{Morpheus}, let alone the dynamic workloads in streaming applications. %This estimation is impossible for streaming applications where the workload is dynamic. Henge instead works with user-facing SLOs that rely on juice and latency.



We present Henge, a system  consisting of the first scheduler to support both multi-tenancy and per-job intents (SLOs) for modern stream processing engines. 
In a cluster of limited resources, Henge continually adapts  to meet jobs' SLOs in spite of other competing SLOs, both under natural system fluctuations, and under input rate changes due to diurnal patterns or sudden spikes. As our goal is to satisfy the SLOs of all jobs on the cluster, Henge must deal with the challenge of allocating resources to jobs continually and wisely. %, but also wisely,and strives
%As our goal is to pack many jobs in one consolidated cluster


%Due to varying input rates, a throughput SLO cannot merely specify an absolute output rate value. Instead, we define a new rate-independent metric for throughput SLOs called {\it juice}, and show how Henge calculates it for arbitrary topologies. Each Henge SLO is specified as a soft {\it utility function} that captures both latency/juice thresholds as well as the fact that the job benefits a little even  if the SLO threshold is not met (e.g., if latency is just above SLO threshold). A utility function  maps each job's current performance  to a value that can be compared across jobs. Henge then attempts to maximize total cluster utility achieved by all jobs in the cluster. 

%At its core, Henge decides wisely how to change allocations of resources to jobs (or rather their basic units, operators) using a new {\it state machine} approach. Our state machine is unique because it is {\it online} in nature: it takes one step at a time, evaluates it, and then moves forward. This is a good match for unpredictable and quickly-changing scenarios such as stream processing clusters. 



We implemented Henge into Apache Storm, one of the most popular modern open-source stream processing system. Our experimental evaluation uses real-world workloads: Yahoo! production Storm topologies, and Twitter datasets. We show that while satisfying SLOs, Henge prevents non-performing topologies from hogging cluster resources. It scales with cluster size and jobs, and is fault-tolerant.

This paper makes the following contributions: %\fkc{This reads more like a summary of the paper than a list of contributions. Juice especially is given no context. The introduction should be complete in itself and should need people to read the summary} \ig{Yes, this is intentional. We are only introducing terms like juice and not using them, so it is ok to defer the definition to.. the next section.}
\squishlist
    \item We present the design of the Henge system and its state machine that manages resource allocation on the cluster.  
    \item We define a new throughput SLO metric called ``juice" and present an algorithm to calculate it.
    \item We define the structure of SLOs using utility functions. 
   % \item We present Henge's state machine that manages resource allocation in the cluster.
    \item We present implementation details of Henge's integration into Apache Storm.
    \item We present evaluation of Henge using real workloads.
\squishend
    %\item We address the problem of capturing throughput SLOs in an input rate-independent way by defining a new metric called {\it juice}.
    %\item We specify an SLO as a soft {\it utility function} that captures both latency/juice thresholds as well as the fact that the job benefits a little even  if the SLO threshold is not met (e.g., if latency is just above SLO threshold). A utility function  maps each job's current performance  to a value that can be compared across jobs. Henge then attempts to maximize total cluster utility achieved by all jobs in the cluster. 
    %\item At its core, Henge decides wisely how to change allocations of resources to jobs (or rather their basic units, operators) using a new {\it state machine} approach. Our state machine is unique because it is {\it online} in nature: it takes one step at a time, evaluates it, and then moves forward. This is a good match for unpredictable and quickly-changing scenarios such as stream processing clusters. \ig{we could also call our approach as ``myopic''. just an idea.}
    
    %\item Specifies each job's SLO  as a mathematical function that maps its behavioral metrics (e.g., latency, throughput) to a {\it utility} value. This {\it utility function} effectively captures both SLO thresholds and job priorities. Then, it continuously monitors the performance of all topologies.
    %\item Adapts the resource allocation of topologies at runtime if they are not meeting their SLO. Henge transfers resources among jobs only if this results in an increase in the  system's utility. 
     %\item Proposes a novel metric called \emph{juice} that allows users to express throughput SLOs as a function of the input rate, regardless of the operations that are carried out per operator and the shape of the job DAG.


%\item We describe implementation details of how Henge is implemented in Apache Storm, the most popular modern open-source stream processing system. 
%\item We present experimental evaluation of Henge using real-world workloads: Yahoo! production Storm topologies, and Twitter datasets. 
%\item We show that Henge meets SLOs under time-variant input rates. Additionally we show Henge prevents non-performing topologies from continuing to hog cluster resources. It scales with cluster size and jobs, and is fault-tolerant.
 
 
 
%In a multi-tenant cluster, it is the scheduler's goal to manage resources to bring and maintain the system in a state that maximizes SLO satisfaction across the cluster. Because the intent is to pack many jobs in the same cluster, the scheduler must deal with the challenge of {\it moving} resources among jobs continually, but also wisely.



%Such wise policies need to determine which operators (fundamental computation units in the stream processing topology)  are bottlenecked and make efforts to alleviate congestion in them. Conversely, they must also reduce the amount of resources allocated to over-provisioned operators. This adaptation of resource allocation to operators must continue not just with workload pattern changes, but also as system behavior fluctuates naturally.



 
 %Henge allows jobs to specify either a latency SLO, or a throughput SLO\footnote{ Hybrid SLOs with both latency and throughput are also possible.}. Time-sensitive jobs (e.g., those related to an ongoing ad campaign) are latency-sensitive while longer running jobs (e.g., sentiment analysis of trending topics) typically have throughput SLOs. Support for a multi-tenant cluster with SLOs eliminates the need for over-provisioning. Instead of the de facto style today of statically partitioning a cluster for  jobs, consolidation makes the cluster shared, more effective, and cost-efficient. 




\begin{comment}
\begin{table}[]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Multi-tenant Schedulers & Workload Type & Adaptivity & Reservation & Resource Usage Profiling & SLO Support \\ \hline
Mesos~\cite{mesos} & General & \xmark & \cmark & ? & \xmark \\ \hline
YARN~\cite{yarn} & General & \xmark & \cmark & ? & \xmark \\ \hline
Henge & Stream & \cmark & \xmark & \cmark & \cmark \\ \hline
Rayon~\cite{curino2014reservation} & Batch & ? & \cmark & ? & \cmark \\ \hline
Omega~\cite{Schwarzkopf:2013:OFS:2465351.2465386} & ? & ? & ? & ? & \cmark \\ \hline
Borg~\cite{verma2015large} & ? & ? & ? & \cmark & \cmark \\ \hline
\end{tabular}%
}
\caption{A comparison between Henge and Existing Schedulers.}
\label{henge-comparison}
\vspace{-1em}
\end{table}
\end{comment}

\begin{comment}
\begin{figure}[ht]
	\vspace{-0.2cm}	
	\begin{center}
		\includegraphics[width=1.0\columnwidth]{figures/same-step.pdf}
		\caption{Two runs of the same topology (on 10 machines) being given the same additional computational resources (28 threads, i.e., executors (Section~\ref{resource-reallocation})).}% 
		\vspace{-0.3cm}	
		\label{same-step}
	\end{center}

\end{figure}

\emph{State Exploration: } Moving resources in a live cluster is a challenging undertaking. 
It entails a state space exploration where every step has both: 1) a significant {realization cost}, because moving resources takes time and affects jobs, and 2) a {convergence cost}, since the system needs a while to converge to steady state after a step. One of our first attempts at designing Henge was to predict latency and throughput gains as a function of resources added, and  use state exploration based on these runtime models. However such prediction is complex and often turns out to be inaccurate  for stream processing systems.  Fig.~\ref{same-step} shows two runs of the same Storm job on 10 machines. In both runs we gave the job equal additional thread resources (28 threads) at t=910 s --  only in  run 1 does latency stabilize, whereas in run 2 it drops to a lower value.  This is due to differing CPU resource consumptions across the runs. More generally, we find that natural fluctuations occur commonly in an application's throughput and latency; left to itself an application's performance changes and degrades gradually over time. Putting all of this  together, we concluded that profiling and runtime modeling would be an infeasible approach. The same observation has been made in other areas like \cite{Morpheus}. 

\end{comment}

==> henge-arxiv 2/text/02-design-overview.tex <==
% \vspace{-0.3cm}
\section{Henge Summary}
\label{summary}

%\subsection{Henge Goals}

%\subsection{Henge Summary}



%Henge allows a developer  to set a per-job SLO that captures the latency and/or throughput intent for their job. The underlying Henge scheduler  has three responsibilities: %\ig{removing this list, to bring the contributions further up front and to maintain flow from the previous section.}

%\begin{enumerate}
	%\item {\bf Monitoring and Detection} to discover which jobs are unable to meet their respective SLOs. %    (Section~\ref{juice})
	%\item {\bf Exploration and Prioritization } to decide which job to give resources, so that achieved system utility is maximized (Section~\ref{policy})
	%\item {\bf Backtracking} to correct mis-steps in the exploration. (Sections~\ref{reduction} and~\ref{reversion}) 
%\end{enumerate}


    %needs to navigate the enormous and unpredictable state space of allocating operators (fundamental computation units in the stream processing topology) to cluster resources. This state space is not predictable or amenable to state space search strategies: even a system 

 %Henge specifies each job's SLO  as a mathematical function that maps its behavioral metrics (e.g., latency, throughput) to a {\it utility} value. This {\it utility function} effectively captures both SLO thresholds and job priorities. The utility function creates a soft SLO, and the function's monotonicity means that the closer the job is to achieving its SLO, the higher its achieved utility. Our approach of using utilities in fact creates a weak form of Pareto efficiency~\cite{wiki:pareto-efficiency} in a system where jobs compete for resources: Henge attempts to maximize the total utility summed across all jobs, and transfers resources among jobs only if the system's utility rises. 


%Due to varying input rates, a throughput SLO cannot merely specify an absolute output rate value. Instead, we define a new rate-independent metric for throughput SLOs called {\it juice}, and show how Henge calculates it for arbitrary topologies. Each Henge SLO is specified as a soft {\it utility function} that captures both latency/juice thresholds as well as the fact that the job benefits a little even  if the SLO threshold is not met (e.g., if latency is just above SLO threshold). A utility function  maps each job's current performance  to a value that can be compared across jobs. Henge then attempts to maximize total cluster utility achieved by all jobs in the cluster. 

%At its core, Henge decides wisely how to change allocations of resources to jobs (or rather their basic units, operators) using a new {\it state machine} approach. Our state machine is unique because it is {\it online} in nature: it takes one step at a time, evaluates it, and then moves forward. This is a good match for unpredictable and quickly-changing scenarios such as stream processing clusters.

We now summarize key ideas behind our contributions. %the paper's

\noindent{\bf Juice:} As input rates can vary over time, it is infeasible for a throughput SLO to merely specify a desired absolute output rate value. Instead, we define a new {\it input rate-independent} metric for throughput SLOs called {\it juice}.  We show how Henge calculates juice for arbitrary topologies (Section~\ref{juice}). %This allows users to set throughput SLOs as a function of input rate.

Juice lies in the interval [0, 1] and  captures the ratio of processing rate to input rate--a value of 1.0 is ideal and implies that the rate of incoming tuples equals rate of tuples being processed by the job. Throughput SLOs can then contain a minimum threshold for juice, making the SLO independent of input rate. We consider processing rate instead of output rate as this generalizes to cases where tuples may be filtered (thus they affect results but are never outputted themselves).% }


\noindent{\bf SLOs: } A job's SLO can capture either latency or juice (or a combination of both). The SLO contains: a) a threshold (min-juice or max-latency), and b) a {\it utility function}, inspired by soft real-time systems \cite{K11}.  The utility function maps current achieved performance (latency or juice) to a value which  represents the benefit to the job, even if it does not meet its SLO threshold. The function thus captures the developer intent that a job  attains full ``utility'' if its SLO threshold is met and partial benefit if not. We support monotonic utility functions: the closer the job is to its SLO threshold, the higher its achieved maximum possible utility. (Section~\ref{job-utilities}).% 


%to ensure users' requests are fulfilled. However, deriving correct resource requirements for jobs is not a straight-forward task~\cite{Morpheus}. In addition, under a constantly changing real-time streaming workload, it is unrealistic for users to provide an estimate of the ideal usage of resource for every variation of the workload. Therefore, Henge does not rely on users' estimation of resource consumption, but instead works with user-facing SLOs such as juice.

%Henge measures throughput relatively by calculating the processing rate of tuples compared to the input rate. We describe an algorithm in Section~\ref{juice} to calculate this metric, called juice. A job's SLO specifies a threshold and a priority, and these are used to create a utility function that maps achieved performance (latency or throughput) to a utility value. Henge attempts to maximize total achieved utility summed across all jobs. It does so by finding SLO-missing topologies, then their congested operators, and gives the operators thread resources according to their  congestion level. Our approach of using utilities in fact creates a weak form of Pareto efficiency~\cite{wiki:pareto-efficiency} in a system where jobs compete for resources: Henge attempts to maximize the total utility summed across all jobs, and transfers resources among jobs only if the system's utility rises.

%\noindent

%Henge's technique attempts to satisfy all jobs' SLOs when the cluster is relatively less packed. When the cluster becomes packed, jobs with higher  priority automatically get more resources as this leads to higher maximum utility for the organization. 


%Further, we postulate that specifying a throughput SLO as an absolute rate is infeasible because the input rate of data being ingested into a job may change over time (e.g., a job ingesting tweets to calculate hashtag counts will show spikes and diurnal variations). Instead, Henge uses a {\it relative} metric called {\it juice} to track throughput. Juice is loosely calculated by the ratio of the processing rate to the input rate and lies in the interval [0, 1].  Throughput SLOs can then be specified via a minimum threshold for juice, and this  makes the SLO independent of input rate. A juice value of 1.0 is ideal and implies that the rate of incoming tuples is the same as the rate of tuples being processed by the topology.% }



 \noindent\textbf {State Space Exploration: }  At its core, Henge decides wisely how to change resource allocations of jobs (or rather of their basic units, operators) using a new {\it state machine} approach (Section~\ref{policy}). Our state machine is unique as it is {\it online} in nature: it takes one step at a time, evaluates its effect, and then moves on. This is a good match for unpredictable and dynamic scenarios such as modern stream processing clusters.
 
 %Moving resources in a live cluster is challenging. It entails a state space exploration where every step has both: 1) a significant {realization cost}, because moving resources takes time and affects jobs, and 2) a {convergence cost}, since the system needs a while to converge to steady state after a step.  Thus, Henge adopts a cautious online approach where next-steps are considered wisely, a step is initiated, the system is allowed to converge, and then the next prospective step is considered (and so on). 
 
 %Henge uses a state machine to explore the state space of which jobs (and their operators) should get how much resources. 
 
 The primary actions in our state machine are: 1) Reconfiguration (give resources to jobs missing SLO), 2) Reduction (take resources away from overprovisioned jobs satisfying  SLO), and 3) Reversion (give up an exploration path and revert to past high utility configuration). Henge  takes these actions  wisely. Jobs are given more resources as a function of the amount of congestion they face. Highly intrusive actions like reduction are minimized in number and frequency. %Small marginal gains in a job's utility lead to it being precluded from reconfigurations in the near future. 
 
 \noindent{\bf Maximizing System Utility: } Design decisions in Henge are aimed at  converging each job quickly to its maximum achievable utility in a minimal number of steps.
Henge attempts to maximize total achieved utility summed across all jobs. It does so by finding SLO-missing topologies, then their congested operators, and gives the operators thread resources according to their  congestion levels. Our approach creates a weak form of Pareto efficiency~\cite{wiki:pareto-efficiency}; in a system where jobs compete for resources, Henge transfers resources among jobs only if this will cause the system's utility to rise. % of using utilities


%Henge's technique attempts to satisfy all jobs' SLOs when the cluster is relatively less packed. When the cluster becomes packed, jobs with higher  priority automatically get more resources as this leads to higher maximum utility for the organization. 



\noindent\textbf {Preventing Resource Hogging:} Topologies with stringent SLOs may try to take over all the resources of the cluster.  To mitigate this, Henge  prefers giving resources to those topologies that: a) are farthest from their SLOs, and b) continue to show utility improvements due to recent Henge actions. This spreads resource allocation across all wanting jobs and prevents starvation and resource hogging.




%The rest of the paper is organized as follows: Section~\ref{background} presents a brief summary of background while Section~\ref{system-design} discusses the essentials of Henge design: how utilities are set (Section~\ref{job-utilities}), how Henge chooses operators for resource allocation (Section~\ref{congestion}) and wisely explores the state space (Section~\ref{policy}). We describe the goals of juice and its computation in Section~\ref{juice}. The implementation of Henge is discussed in Section~\ref{system-architecture}. We conclude after evaluation (Section~\ref{evaluation}) and a discussion of related work (Section~\ref{related-work}).


\begin{table*}[ht!]
	\small
	\begin{tabular}{p{0.09\linewidth} p{0.4\linewidth} p{0.45\linewidth}}%[h]{c|c|c} 
		\toprule
		\textbf{Business} & \textbf{Use Case} & \textbf{SLO Type} \\
		\midrule%\hline
		\multirow{2}{6em}{The Weather Channel} & Monitoring natural disasters in real-time & Latency e.g., a tuple must be processed within 30 seconds \\ 
		& Processing collected data for forecasts 
		& Throughput e.g, processing data as fast as it can be read \\%from the data source
		\midrule
		\multirow{2}{7em}{WebMD}  & Monitoring blogs to provide  real-time updates & Latency e.g., provide updates within 10 mins  \\ 
		& Search Indexing & Throughput e.g., index all new  sites at the rate they're found  \\
		\midrule
		\multirow{2}{7em}{E-Commerce Websites}  & Counting ad-clicks & Latency e.g., click count should be updated every second  \\ 
		&  Alipay uses Storm to process 6 TB logs per day & Throughput e.g., process logs at the rate of generation \\
		\bottomrule
	\end{tabular}
	\normalsize
	\vspace{-0.5em}
	\captionof{table}{\bf Stream Processing Use Cases and Possible SLO Types.}
	\label{table-slos}
	\vspace{-1.5em}
\end{table*}

The rest of the paper is organized as follows: Section~\ref{background} presents  background. Section~\ref{system-design} discusses core Henge design: SLOs and utilities (Section~\ref{job-utilities}), operator congestion (Section~\ref{congestion}), and the state machine (Section~\ref{policy}). Section~\ref{juice} describes juice and its calculation. Implementation details are in Section~\ref{system-architecture}, evaluation in Section~\ref{evaluation}, and related work in Section~\ref{related-work}. We conclude in Section~\ref{conclusion}.

==> henge-arxiv 2/text/03-stream-processing-overview.tex <==
\vspace{-0.2cm}
\section {Background}
\label{background}
% \vspace{-0.2cm}

A stream processing job can be logically interpreted as a \emph{topology}, i.e., a directed acyclic graph of \emph{operators} (we sometimes use the Storm term ``bolt"). We use the terms job and topology interchangeably in this paper. An operator is a logical processing unit that applies user-defined functions on a stream of \emph{tuples}. Source operators (called spouts) pull input tuples while sink operators spew output tuples. The sum of output rates of sinks in a topology is its {\it output rate}, while the sum of all spout rates is the {\it input rate}. Each operator is  parallelized via multiple \emph{tasks}. Fig.~\ref{simple-topology} shows a topology with one spout and one sink. 


\begin{figure}[!h]
\vspace{-0.2cm}
	\begin{center}
		\includegraphics[width=0.5\textwidth]{figures/simple-topology.pdf}
	\end{center}
	\vspace{-1.5em}
	\caption{{\bf Sample Storm topology.} \it Showing tuples processed per unit time. Edge labels indicate number of tuples sent out by the parent operator to the child. (Congestion described in Section~\ref{juice}.) }%\fkc{bolt to operator}
	\label{simple-topology}
	\vspace{-0.2cm}
\end{figure}

 We consider long-running stream processing topologies with a continuous operator model. A topology is run on one or more worker processes, which in turn instantiate {\it executors} (threads), which run tasks specific to one operator.  An operator processes  streaming data one tuple at a time and forwards the tuples to the next operators in the topology.  Systems that follow such a model include Apache Storm~\cite{toshniwal2014storm}, Heron~\cite{heron}, Flink~\cite{flink} and Samza~\cite{samza}. 

\noindent\textbf{Definitions:} %Users running topologies care about the \emph{latency} and \emph{throughput} of their jobs. 
% The latency of a tuple is the time for it to enter  the topology from the source to producing an output result on any sink.  
The latency of a tuple is the time between it entering  the topology from the source, to producing an output result on any sink.  A {\it topology's latency} is then the average of tuple latencies, measured over a period of time. A {\it topology's throughput} is  the number of tuples it processes per unit time. 

A {\it Service Level Objective (SLO)}~\cite{wiki:SLO} is a customer topology's requirement, in terms of latency and/or throughput. 
Table~\ref{table-slos} shows several real streaming applications~\cite{alipay-stats}, and the latency or throughput SLOs they may require.  


Other examples of latency-sensitive jobs include applications that perform real-time analytics or real-time natural language processing, provide moderation services for chat rooms, count bid requests, or calculate real-time trade quantities  in stock markets. Examples of throughput-sensitive application include jobs that perform incremental checkpointing, count online visitors, or perform sentiment analysis.





==> henge-arxiv 2/text/05-system-design.tex <==
\vspace{-0.5em}
\section{System Design}
\label{system-design}

We discuss Henge's utility functions (Section~\ref{job-utilities}), congestion metric (Section~\ref{congestion}), and its state machine (Section~\ref{policy}). 



\vspace{-0.25cm}
\subsection{SLOs and Utility Functions}
\label{job-utilities}




Each topology's SLO contains: a) an SLO threshold (min-juice or max-latency), and b) a {utility function}. 
%Each job's (topology's) SLO contains a utility function. 
The utility function maps the current performance metrics of the job (i.e. its SLO metric) to a \emph{current} utility value. This approach abstracts away the type of SLO metric each topology has, and allows the scheduler to compare utilities across jobs. %This is the utility value a topology currently provides, as a function of where it is w.r.t. its SLO threshold.
%Different users may have different SLO metrics for their jobs, given the nature of their application. For instance, some users may be concerned with end-to-end latency of the topology and others may be concerned with throughput. The metric we use in place of throughput is juice (details in Section~\ref{juice}). 

%This allows Henge to compare the performance of topologies with each other and  enables users of Henge to state the SLOs of their topologies in terms of any measurable metric they choose as long they also provide its utility function. 



Currently, Henge supports both latency and throughput metrics in the SLO. Latency was defined in Section~\ref{background}. 
%The former is the end-to-end latency suffered by tuples, from their moment of ingestion into the topology until the point of exit form a sink operator. 
For throughput, we use a new SLO metric called juice which we  define concretely later in Section~\ref{juice} (for the current section, an abstract throughput metric suffices). %Henge also supports a combination of these SLO metrics.


%  Recall that juice is a relative measure of throughput found by calculating the processing rate of tuples compared to the input rate.

%\fkc{juice --> a throughput metric, later refer back., eqn 1 with juice...}

%  When the  SLO threshold cannot be satisfied, the job still desires {\it some} level of performance close to the threshold. Hence, utility functions must be monotonic--for a latency SLO job, the utility function must be monotonically non-increasing as latency rises, while for a throughput SLO job, it must be monotonically non-decreasing with throughput. 

 When the  SLO threshold cannot be satisfied, the job still desires {\it some} level of performance close to the threshold. Hence, utility functions must be monotonic--for a job with a latency SLO, the utility function must be monotonically non-increasing as latency rises, while for a job with a throughput SLO, it must be monotonically non-decreasing as throughput rises. 

Each utility function has a {\it maximum utility} value, achieved only when the SLO threshold is met e.g.,  a job with an SLO threshold of 100 ms would achieve its maximum utility  only if its current latency is below 100 ms. As latency grows above 100 ms, utility can fall or plateau but can never rise.




The {maximum  utility value} is based on job priority.  For example, in Fig.~\ref{utility}a, topology T2 has twice the priority of T1, and thus has twice the maximum utility (20 vs. 10). 




Given these requirements, Henge is able to allow a wide variety of shapes for its utility functions including: linear, piece-wise linear, step function (allowed because utilities are monotonically non-increasing instead of monotonically decreasing), lognormal, etc. Utility functions do not need to be continuous. All in all, this offers users flexibility in shaping utility functions according to individual needs. %such that it maps the topology's performance exactly to utility values that reflect the true gain. % from having achieved that performance.



%This formulation (non-increasing instead of strictly increasing) is needed so the utility function can {\it plateau out} when the SLO threshold is reached. The plateau is the maximum achievable utility for that job. For instance, a job with an SLO threshold of 100 ms would achieve a constant (maximum) utility value only if its current latency is below 100 ms. At higher latencies,  but lower utility at higher latencies. Similarly only when the achieved throughput metric is above the SLO threshold is the utility maxed out.  %A job with a throughput SLO threshold of 1000 tuples per second would specify a constant utility value for all juice values above  1000 tuples per second  but lower utility values below. \ig{you can't say this as absolute is not our throughhput metric!}



%\ig{how does this work? you are using juice in these equations and text, but the juice sections have not come yet. }

%\fkc{replace figure} \ig{why replace? lgtm.} \fkc{Because the original said juice, not throughput}


\begin{figure}[ht!]
% 	\vspace{-0.2cm}
	\begin{center}
		\includegraphics[width=1.0\columnwidth]{figures/utilities/throughput-SLO.pdf}
	\end{center}
	\vspace{-0.4cm}
	\caption{ {\bf Knee Utility functions}. \it  (a) Throughput SLO utility, (b) Latency SLO utility.  } %Used in our implementation. Other utility functions are possible. 
	\vspace{-0.4cm}
	\label{utility}
\end{figure}

The concrete utility functions used in our Henge implementation are {\it knee} functions, depicted in Fig.~\ref{utility}. A knee function has two  pieces: a plateau beyond the SLO threshold, and a sub-SLO part for when the job does not meet the threshold. Concretely, the  achieved utility for jobs with throughput and latency SLOs respectively, are:%, for juice and latency SLOs respectively, the current utility of a job is:





\vspace{-2em}

\small
\begin{center}
	\begin{equation} 
	\frac{\tt Current\ Utility}{Job\ Max\ Utility} = min(1, \frac{Current\ Throughput\ Metric}{SLO\ Throughput\   Threshold})
%	 \textbf{this is min of 1, and frac}
	\label{eq:5}
	\end{equation}
	\vspace{-0.5em}
	\begin{equation} 
	\label{eq:6}
	\frac{\tt Current\ Utility}{Job\ Max\ Utility} = min(1, \frac{SLO\ Latency\ Threshold}{Current\ Latency}) %\times Job\_Max\_Utility
	\end{equation}
\end{center}
% \vspace{-0.5em}
\normalsize

The sub-SLO is the last term inside ``min". 

For throughput SLOs, the sub-SLO is linear and arises from the  origin point. For latency SLOs, the sub-SLO is hyperbolic ($y \propto \frac{1}{x}$), allowing increasingly smaller utilities as latencies rise. Fig.~\ref{utility} shows a throughput SLO  (Fig.~\ref{utility}a) vs. latency SLO  (Fig.~\ref{utility}b). 

%\ig{very meandering paragraph}It is possible for users to set very high utility values for a particular job, thereby giving it higher priority. This may lead to a situation where the majority of cluster resources are allocated to the high priority job. This is  acceptable in the case of Henge as it assumes that the scheduler is used internally within one organization, where users do not want to step on each other, and thus makes no guarantees about fairness. Its goal is to maximize the total utility of the topology and giving resources to the highest priority job may be one way to do that. One way to add fairness is to use utility functions to capture the dollar cost of running a job in a multi-tenant cluster with monetary contracts. Then, lower utilities translate to lower payment from the customer to the provider.  Utility functions are thus useful in Service Level Agreements (SLAs). 

We envision Henge to be used internally inside companies, hence job priorities are set in a consensual way (e.g., by upper management). The utility function approach is also amenable to use in contracts like Service Level Agreements (SLAs), however these are beyond the scope of this paper.

%\fkc{Alternatively, the scheduler can be used as an internal scheduler within a company where the cluster administrator helps each user set their utilities in accordance with their work priority. This prevents  users from setting very high utility values which may lead to their jobs usurping the resources allocated to other jobs. }





==> henge-arxiv 2/text/06-resource-reallocation.tex <==
% \vspace{-0.1cm}
\subsection{Operator Congestion Metric}
\label{congestion}

A topology misses its SLOs when some of its operators become \emph{congested}, i.e., have insufficient resources. To detect congestion our implementation uses a metric called operator \emph{capacity}~\cite{capacity-metric}.  However, Henge can also use  other existing congestion metrics, e.g.,  input queue sizes or ETP~\cite{xu:16:ic2e}. 



Operator capacity captures the fraction of time that an operator spends processing tuples during a time unit. Its values lie in the range $[0.0, 1.0]$. If an executor's capacity is near 1.0, then it is close to being congested. 

Consider an  executor $E$ that runs several (parallel) tasks of a topology operator. Its capacity   is calculated as:
	 
	  %In Storm, the number of executors that belong to each operator is called its parallelism level~\cite{storm-parallelism-level}. Each executor runs one or more \emph{tasks} of the same operator. The actual work of the operator is performed in the task. The capacity of an operator is the maximum capacity that any of its executors has.
	% Concretely for an executor E:

\vspace{-0.6cm}
\begin{center}
\small

	\begin{equation} \label{eq:3}
	Capacity_{E} =  \frac{{Executed\ Tuples}_{E}\times{Execute\ Latency}_{E}}{Unit\ Time}
	\end{equation}
\end{center}
\vspace{-0.1cm}
\normalsize



\noindent where $Unit\ Time$ is a time window. The numerator multiplies the number of tuples executed in this window and their average execution latency to calculate the total time spent in executing those tuples.  %Dividing with unit time, we obtain the fraction of  time the executor was busy executing these tuples. 
The operator capacity is then the maximum capacity across all executors containing it.




Henge considers an operator to be congested if its capacity is above the threshold of 0.3. This increases the pool of possibilities, as more operators  become candidates for receiving resources (described next). % (described next).

%By choosing the maximum capacity among all executors assigned to the operator, Henge is able to identify the worst case operator bottlenecks in the topology.% \ig{bottleneck is one word, not hyphenated. replace all.}

 %~\footnote{Experimentally, we find that Storm can report capacities > 1, as the value of execute latency is obtained by averaging latency values since the start time of the topology, instead of just the values from the last time window. This is also mentioned in~\cite{capacity-greater-one}.}. 


%Henge mitigates congestion by giving an operator a number of extra threads, proportional to its congestion level. The number of extra threads is given by this equation:
%\vspace{-0.5cm}
%\small
	
%	\begin{center}
%		\begin{equation} 
 %\left(\frac{Current\ Operator\ Capacity}{Capacity\ Threshold}-1
 %\right)  \times 10
%		%\label{extra_resources}
%		\label{eq:executors}
%		\end{equation}
%	\end{center}
%	\normalsize

%We will refer back to this equation when we describe the state machine in the next section.

% \label{resource-reallocation}

%Henge removes congestion in an operator by scaling the number of executors of the operator.% In Storm, the number of executors that belong to each operator is called it's parallelism level~\cite{storm-parallelism-level}. Each executor runs one or more \emph{tasks} of the same operator. The actual work of the operator is performed in the task. 


%scales up the number of threads given to an operator in proportion to its congestion. Concretely, the number of additional threads  is calculated as:

	
	
% 	\vspace{-0.1cm}
	
	%Intuitively, this means that the more congested an operator is, the more threads it gets. This minimizes the number of reconfigurations required to remove congestion from the chosen operator. Once the number of additional executors is determined, Henge proceeds to deploy the new schedule. 


%\ig{why is this our strategy? why is this the best strategyZ?}

 %\ig{rest of para seems repetitious. remove.} Fig~\ref{increase-executors} shows the effect of increasing executors for congested operators  on a topology's performance. Capacity above 0.3 triggers a reconfiguration of a topology. As congestion is resolved by additional executors, the topology's performance improves.
 
 \begin{comment}
\begin{figure}[t]
	\begin{center}	
			\includegraphics[width=0.5\textwidth]{figures/exp107/together.pdf}
	\end{center}
	\vspace{-0.7cm}
	\caption{ Reconfiguration increases operator parallelism level from 4 to 27 executors. The operator's capacity drops corresponding with the performance improvement.
	\fkc{Make a plot of throughput vs latency, and get rid of time and the second Y axis. Can be a bar graph. Put capacity as values on the bars}}
	\label{increase-executors}
	\vspace{-0.5cm}	
\end{figure}	
\end{comment}

==> henge-arxiv 2/text/07-policy_II.tex <==
\subsection{Henge State Machine}
\label{policy}

The state machine (shown in Fig.~\ref{henge-state-machine}) considers all jobs in the cluster as a whole and wisely decides how many resources to give to congested jobs in the cluster and when to stop. The state machine is for the entire cluster, not per job. %A topology is in the converged state if its utility is max (meets its SLO thresholds), otherwise it is in the ``Not Converged" state.

 The cluster is in  the Converged state if and only if either: a) all topologies have reached their maximum utility (i.e., satisfy their respective SLO thresholds), or b) Henge recognizes that no further actions will improve the performance of any topology, and thus it has reverted to the last best configuration. All other states are Not Converged. 
 
 To move among these two states, Henge uses three actions: Reconfiguration, Reduction, and Reversion.
 
 \begin{figure}[h]
	\vspace{-0.1cm}
	\begin{center}
		\includegraphics[width=1\columnwidth]{figures/state-transition-diagram-2.pdf}
	\end{center}
	\vspace{-0.3cm}
	\caption{\bf Henge's State Machine for the Cluster.}%State machine for Henge's scheduling decisions.}
	\label{henge-state-machine}
	\vspace{-0.4cm}
\end{figure}
 
 \subsubsection{Reconfiguration}

In the Not Converged state, a Reconfiguration gives resources to topologies missing their SLO. Reconfigurations occur in {\it rounds} which are periodic intervals (currently 10 s apart).  
In each round, Henge first sorts all topologies missing their SLOs, in descending order of their maximum utility, with ties broken by preferring lower current utility. It then picks the head of this sorted queue to allocate resources to. 
 %This is thus  a topology with the highest maximum (achievable) utility and the lowest current utility. 
 This greedy strategy works best to maximize cluster utility. 

 Within this selected topology, the intuition is to increase each congested operator's resources by an amount proportional to its respective congestion. Henge  uses  the capacity  metric (Section~\ref{congestion}, eq.~\ref{eq:3}) to discover all congested operators in this chosen topology, i.e., operator capacity $>0.3$. It allocates each congested operator an extra number of threads based on the following equation:  
 
%Henge mitigates congestion by giving an operator a number of extra threads, proportional to its congestion level. The number of extra threads is given by this equation:
\vspace{-0.6cm}
	\begin{center}
		\begin{equation} 
		\small
 \left(\frac{Current\ Operator\ Capacity}{Capacity\ Threshold}-1
 \right)  \times 10
		%\label{extra_resources}
		\label{eq:executors}
		\end{equation}
	\end{center}
	\normalsize

%This gives an operator a number of extra threads, proportional to its congestion level.


Henge deploys this configuration change to a single topology on the cluster, and waits for the measured utilities to quiesce (this typically takes a minute or so in our configurations). No further actions are taken in the interim. It then measures the total cluster utility again, and if it improved, Henge  continues its operations in further rounds, in the Not Converged State. If this total utility reaches the maximum value (the sum of  maximum utilities of all topologies), then Henge cautiously continues monitoring the recently configured topologies for a while (4 subsequent rounds in our setting). If they all  stabilize, Henge moves the cluster to the Converged state. % of convergence.

A topology may improve only marginally after being given more resources in a reconfiguration, e.g., utility increases $<5$\%. In such a case, Henge retains the reconfiguration change but skips this particular topology in the near future rounds. This is because the topology may have plateaued in terms of marginal benefit from getting more threads. Since the cluster is dynamic, this black-listing of a topology is not permanent but is allowed to expire after a while (1 hour in our settings), after which the topology will again be a candidate for reconfiguration.
%Thereafter, if there is an observable drop in performance while in the converged state ($> 5\%$), Henge infers that the workload of the topologies may have changed. It moves back to the non-converged state, and starts attempting reconfigurations again. 

As reconfigurations are exploratory steps in the  state space search, total system utility may  decrease after a step. Henge employs two actions called {Reduction} and {Reversion} to handle such cases.

\vspace{-0.1cm}

\subsubsection{Reduction}
\label{reduction}

% If a Reconfiguration improves system utility, the next action will be a Reconfiguration.
If a Reconfiguration causes total system utility to drop, the next action is either a Reduction or a Reversion. Henge performs Reduction if and only if three conditions are  true: (a) the  cluster is congested (we detail below what this means),  (b) there is at least one SLO-satisfying topology, and (c) there is no past history of a Reduction action. %\ig{ verify this please -- if reconfig only drops cluster utility but does not cause congested cluster (majority) then we continue reconfigurations and do not revert. If this statement is untrue, please revise this para and start of Reversion section and state machine description to make them consistent.}


%If a reconfiguration step results in a drop of the total system utility, Henge has two options: continue further reconfigurations, or \fkc{back off}. We back off only if the cluster is congested--we detail how to detect this. %\ig{ verify this please -- if reconfig only drops cluster utility but does not cause congested cluster (majority) then we continue reconfigurations and do not revert. If this statement is untrue, please revise this para and start of Reversion section and state machine description to make them consistent.}

First, CPU load is defined as the number of processes that are running or runnable on a machine~\cite{load}. A machine's load should be $\leq$ number of available cores, ensuring maximum utilization and no over-subscription.  
As a result, Henge considers a machine congested if its CPU load exceeds its number of cores. Henge considers a {\it cluster congested} when it has a majority of its machines congested. 

If a Reconfiguration drops utility and results in a  congested cluster, Henge executes  Reduction to reduce congestion. For all topologies {\it meeting} their SLOs, it finds all their un-congested operators (except spouts) and reduces their parallelism level by  a large amount (80\% in our settings). If this results in SLO misses, such topologies will be considered in future reconfiguration rounds. To minimize intrusion, Henge limits  Reduction to once per topology; this is reset if external factors  change (input rate, set of jobs, etc.).% in order to reduce CPU load.  
%If a  drop in cluster utility is accompanied by an increase in CPU load exceeding the number of  cores for a majority of machines in the the cluster, Henge executes reduction. 

Akin to backoff mechanisms~\cite{jacobson1988congestion}, massive reduction is the only way to free up a lot of resources at once,  
%and reduce over-provisioning, 
so that future reconfigurations may have a positive effect. Reducing threads also decreases their context switching overhead. 
 


%If this massive reduction causes some topologies to miss their SLOs, they  will be reconfigured in future rounds. %At the end, they would have the exact amount of resources they need to satisfy their SLOs. 
%To minimize its intrusive effect, this reduction step is carried out at most once for any given topology; this is reset if external factors  change (input rate, set of jobs, etc.).


Right after a reduction, if the next reconfiguration drops cluster utility again while keeping the cluster congested (measured using CPU load), Henge recognizes that performing another reduction would be futile.  This is a typical ``lockout" case, and  Henge resolves it by performing Reversion. %\ig{original line here was ``while increasing CPU load'' - this was never defined! see commented para.}
% (described next). 


 %\ig{please check if the first sentence in this para is true. this is based on points that Bobby pointed out.} \igc{In Reduction we explicitly chose to reduce threads (executors) rather than  reducing tasks within an operator. This is because of multiple reasons: 1)  reducing the number of tasks would have been more intrusive (requiring reordering of key ranges across tasks in the same operator, e.g., in fields grouping of Storm),  2) reducing number of threads improves batching, and 3) reducing number of threads improves context switching overhead. }\fkc{Tasks cannot be changed during runtime. Code has to changed and recompiled to do that. Bringing up point 2 requires additional explanation of the Disruptor queue which is unnecessary.   I have added 3) above.}
 \vspace{-0.1cm}
\subsubsection{Reversion}
\label{reversion}

If a Reconfiguration drops utility and a Reduction is not possible (meaning that at least one of the conditions (a)-(c) in Section~\ref{reduction} is not true), Henge performs Reversion.
%A Reversion is executed if and only if the previous step was a  Reconfiguration, it dropped utility, and at least one of conditions (a)-(c) in Section~\ref{reduction} are false. % this description is too mechanical 


% or (ii) the previous step was a Reduction, and \ig{what?}. \fkc{A reversion cannot occur after a reduction because we refresh history}

%In its state space search, when Henge finds that its reconfiguration or reduction policies cannot improve utility further, it reverts to the latest configuration that gave the highest system utility in the past. Reversions occur when:

%When Henge is ``stuck" in its state space search it  reverts the cluster back to its best recent configuration (highest past utility).

%Reversions occur when any one of the following conditions is satisfied: % \ig{are these scenarios in addition to or a superset of the scenarios form the previous subsection?}\fkc{a superset. The first item makes it a superset}:
%\ig{these conditions need to be each complete and mutually exclusive from each other.}

%\squishlist

% \item A reconfiguration causes poorer utility, \igc{and a congested cluster,} \ig{? (otherwise this contradicts the first para of Sec 4.3.2)} entailing that it was an unwise decision, or % and the average CPU load (across machines) did not increase. \ig{please rework this to be correct. what is this? increase in CPU load for each  machine? or for cluster, averaged over machines? or for majority of machines? or do you mean keeps cluster congested (see definition above).}.

% \item After a reduction step, the next reconfiguration step drops cluster utility and causes a congested cluster again (majority of machines have CPU load $>$ number of cores). \ig{isn't this the same as the first condition above? if so, replace the first bullet with this one}%, or %\ig{I do not understand the following phrase. Makes no sense. Suggest removing it and ending sentence here},

% \item Henge would like perform a reduction, but there are no SLO-satisfying topologies that can be reduced, or

%\item  A reconfiguration leads to poorer system utility, accompanied by an increase in CPU load. However, a reduction has already been performed for current workload or there are no SLO-satisfying topologies that can be reduced.  

%\item A reconfiguration leads to poorer utility with no correlated increase in CPU load. This entails that the last reconfiguration decision was unwise.

%\squishend


%\squishlist
%\item A reconfiguration leads to poorer system utility, accompanied by an increase in CPU load. However, a reduction has already been performed for current workload or there are no SLO-satisfying topologies that can be reduced. (Cases discussed at the end of Section~\ref{reduction}.)
%\item A reconfiguration leads to poorer utility with no correlated increase in CPU load. This entails that the last reconfiguration decision was unwise.
%\squishend

Henge sorts through its history of Reconfigurations and picks the one that maximized system utility. It moves the system back to this past configuration by resetting the resource allocations of all jobs to values in this past configuration and moves to the Converged state. Here, Henge essentially concludes that it is impossible to further optimize cluster utility, given this workload. Henge maintains this configuration until changes like further SLO violations occur, which necessitate reconfigurations.% The only hope is if the workload itself were to change. 

%\igc{It moves to the Converged State.} \ig{is this correct? to be consistent with the state machine and its description earlier in this section.} % In the dire situation of a 

%all jobs back to their allocations in best recent %recent
%resource allocation (that maximized its uility). % \ig{best or recent? what if the history of past utilities is (oldest to newest) 55, 60, 45, 40, 40, 40, 40, 52, 50, 30. Will it go to 52 or 60?} \fkc{60. (This is not a problem because we refresh history if the workload changes. In fact, the set of utilities provided here shouldn't even be possible because Henge does a revert if a reconfiguration drops the total utility by more than 5\%)}. 


%This allows the cluster to run in this chosen configuration and reaches the state of convergence, where the system maintains a stable state (until further changes like further SLO violations which reactivate Henge). 

%\ig{Not clear if this means that Henge remains stuck until some outside parameter changes. That is, does Henge continue taking further actions?}\fkc{Henge does stay in this state without making further changes until an external parameter changes. An alternative to this would be to explore other resource bottlenecks like memory etc at this point. }

%At this point, Henge policy cannot provide better system utility. 
If a large enough drop ($>5 \%$) in utility occurs in this Converged state (e.g., due to new jobs, or input rate changes), Henge infers that as reconfigurations cannot be a cause of this drop, the workload of topologies must have changed. As all past actions no longer apply to this change in behavior, Henge  forgets all history of past actions and moves to the Not Converged state. This means that in future reversions, forgotten states will not be available. This reset allows Henge to start its state space search afresh. %; this decision allows Henge to only revert to recent good states.

==> henge-arxiv 2/text/08-discussion.tex <==
% \vspace{-0.2cm}
\subsection{Discussion}
\noindent{\bf Online vs. Offline State Space Search:} 
%Resources must be moved carefully in a cluster to ensure that running jobs are minimally affected and the system converges quickly after a step. 
Henge prefers an online state space search. In fact, our early attempt at designing Henge was to perform offline state space exploration (e.g., through simulated annealing), by measuring SLO metrics (latency, throughput) and using analytical models to predict their relation to resources allocated to the job.
%predict latency and throughput gains as a function of resources. Our approach was to use analytical models so that we could use offline state space exploration like simulated annealing). 


\begin{figure}[ht]
	\vspace{-0.3cm}	
	\begin{center}
		\includegraphics[width=1.0\columnwidth]{figures/same-step.pdf}
		\caption{{\bf Unpredictability in Modern Stream Processing Engines:} \it Two runs of the same topology (on 10 machines) being given the same extra computational resources (28 threads, i.e., executors) at 910 s, react differently.}% 
		\vspace{-0.4cm}	
		\label{same-step}
	\end{center}

\end{figure}


The offline approach turned out to be impractical. Analysis and prediction is complex and often turns out to be inaccurate  for stream processing systems, which are very dynamic in nature. (This phenomenon has also been observed in other distributed scheduling domains, e.g., see ~\cite{automatic-tuning,Morpheus,ousterhout2017monotasks}.)  
We show an example in Fig.~\ref{same-step}. The figure shows two runs of the same Storm job on 10 machines. In both runs we gave the job equal additional thread resources (28 threads) at t=910 s. Latency drops to a lower value in run 2, but only stabilizes in run 1. %Only in  run 1 does latency stabilize, whereas in run 2 it drops to a lower value. 
This is due to differing CPU resource consumptions across the runs. More generally, we find that natural fluctuations occur commonly in an application's throughput and latency; left to itself an application's performance changes and degrades gradually over time. We observed this for all our  actions: reconfiguration, reduction, and reversion. Thus, we concluded that online state space exploration would be more practical.% a better approach. %Putting all of this  together

%\igc{\noindent{\bf Tail Latencies: } Henge can be extended to tackle tail latencies (e.g., 95th percentile, or 99th percentile). In SLOs, average latency can be replaced with a tail latency metric (utility functions remain unchanged). The scheduler can be configured to measure and react to tail latency. }

%\igc{
\noindent{\bf Tail Latencies: } Henge can also admit SLOs expressed as tail latencies (e.g., 95th percentile, or 99th percentile). Utility functions are then expressed in terms of  tail latency and the state machine remains unchanged.%. The scheduler uses the same state machine, but reacts to tail latency instead of average latency.% with average latency replaced with tail latency.
%}

%Therefore, Henge policy is based on an online state machine, where each step is considered carefully before deployment and is evaluated afterwards to ensure efficacy. 


\noindent{\bf Statefulness, Memory Bottlenecks: } The common case among topologies is stateless operators that are CPU-bound, and our exposition so far is thus focused. Nevertheless, Henge gracefully handles stateful operators and memory-pressured nodes (evaluated in Sections~\ref{sec:stateful_expts}, \ref{sec:memory-utilization}).

%Other works by Ousterhout et al \cite{ousterhout2015making} have noted that cluster systems are typically CPU-bottlenecked, and that memory and network limits can be improved via optimizations and better programming. Nevertheless, Henge's approach could be generalized to cover multiple resources types (however this is beyond our scope here). 

%\noindent{\bf Statefulness: } Henge generalizes to stateful topologies. Stateful operators are rarer than stateless operators. Nevertheless, in such cases state is handled orthogonally by the operators, even when Henge is scaling it out or in. (Experiments in Section~\ref{sec:stateful_expts}.)%. When the Henge scales the operator out or in, the operator's semantics ensure correctness.

%\noindent{\bf Memory Bottlenecks:}
%Henge largely accounts for CPU load and bottlenecks. 
%CPU bottlenecks. 
%However, our system also keeps memory low (Experiments in Section~\ref{sec:memory-utilization}.)
%also alleviates memory bottlenecks (Experiments in Section~\ref{sec:memory-utilization}.) %\fkc{[insert plot here]}. \ig{don't insert plot here. refer to exptl. section number}


%\fkc{State here that statefulness also works}

==> henge-arxiv 2/text/09-juice.tex <==
%\vspace{-0.5cm}
\section{Juice: Definition and Algorithm}
\label{juice}

%\fkc{Justify more why juice is important in place of throughput}
	As described in Section~\ref{introduction}, we wish to design a throughput metric (for use in throughput SLOs), in a way that is independent of input rate. Henge uses a new metric called {\it juice}. Juice defines what fraction of the input data is being processed by the topology per unit time. It lies in the interval [0, 1], and a value of 1.0 means all the input data that arrived in the last time unit has been processed. Thus, the user can set throughput requirements as a percentage of the input rate (Section~\ref{job-utilities}), and Henge subsequently attempts to maintain this even as input rates change.
	
	
	%Essentially, juice captures what fraction of the input data is being processed by the topology. %It allows us to: 1) abstract away throughput SLO requirements in a way that is independent of absolute input rate, and 2) track whether congestion is occurring inside a  topology (job). %Our design of the juice metric is based on three principles: 
Any algorithm that calculates juice should be: %satisfy three requirements:

\noindent{\it 1. Code Independent:} It should be independent of the operators' code, and should be calculate-able by only considering the number of tuples generated by  operators.

\noindent{\it 2. Rate Independent:} It should be independent of input  rates. %abstract away throughput SLO requirements in a way that is independent of absolute input rate.

%It should be independent of the input rate of the topology, which may vary over time. %\ig{repetitious; already mentioned in first para of this section. remove?}

\noindent{\it 3. Topology Independent:} It should be independent of the shape and structure of the topology. %, and should hold across all possible shapes, e.g., diamond, star, linear, trees, and production shapes.



\noindent{\bf Juice Intuition: } Overall, juice is formulated to reflect the {\it global} processing efficiency of a topology. 
 We define per-operator contribution to juice as the proportion of input passed in originally \emph{from the source} that the operator processed in a given time window. This reflects the impact of that operator \emph{and} its upstream operators, on this input. The juice of a topology is then the normalized sum of  juice values of all its sinks. 

\noindent{\bf Juice Calculation: }Henge calculates juice in configurable windows of time (unit time). We define {\it source input} as the tuples that arrive at the input operator in a unit of time. For each operator $o$ in a topology that has $n$ parents, we define $T_{o}^{i}$ as the total number of tuples sent out from its ${i}^{th}$ parent per time unit, and $E_{o}^{i}$ as the number of tuples that operator $o$ executed (per time unit), from those received from parent $i$.

The per-operator contribution to juice, $J_{o}^{s}$, is the proportion of source input {\it sent} from source $s$ that operator $o$ received and processed. 
Given that  $J_{i}^{s}$ is the juice of $o$'s $i^{th}$ parent, then $J_{o}^{s}$ is: 

\vspace{-1.0cm}
\small
\begin{center}
\begin{equation} \label{eq:1}
J_{o}^{s} = \sum\limits_{i=1}^n \left( J_{i}^{s} \times \frac{E_{o}^{i}}{T_{o}^{i}} \right)
\end{equation}
\end{center}
\vspace{-0.2cm}
\normalsize

A spout $s$ has no parents, and its juice: $J_{s}=\frac{E_{s}}{T_{s}} = 1.0$ .

In eq.~\ref{eq:1}, the fraction $\frac{E_{o}^{i}}{T_{o}^{i}}$ reflects the proportion of tuples an operator received from its parents, and processed successfully.  If no tuples waiting in queues, this fraction is equal to 1.0. By multiplying this value with the parent's juice we accumulate through the topology the effect of all upstream operators. 

%\ig{Please verify} 
We make two important observations. In the term $\frac{E_{o}^{i}}{T_{o}^{i}}$,  it is critical to take the denominator as the number of tuples {\it sent} by a parent rather than received at the operator. This allows juice: a)  to account for data splitting at the parent (fork in the DAG), and b) to be reduced by  tuples dropped by the network. The numerator is the number of {\it processed} tuples rather than the number of output tuples -- this allows juice to generalize to operator types whose processing  may drop tuples (e.g., filter).


Given all operator juice values, a topology's juice can be calculated by normalizing w.r.t. number of sources:
\vspace{-0.5cm}
\begin {center}
\begin {equation} \label{eq:2}
\frac{\sum\limits_{Sinks\ s_{i},\  Sources\ s_{j}}(J_{s_{i}}^{s_{j}} )}{ { Total \ Number \ of \ Sources}}
%\normalsize
\end {equation}
\end {center}
\vspace{-0.1cm}


%\ig{DO NOT use normalsize. It is shrinking the font.}

%If there are two or more source operators in the topology, the numerator may be greater than 1.0. 
If no tuples are lost in the system, the numerator sum is equal to the number of sources. To ensure that juice stays below 1.0, we normalize the sum with the number of sources. %In Example 1 (Fig. \ref{simple-topology}), $Juice = J_{sink}^{s} = 0.875 $.
%\ig{please double check all calculations.} 
%We note (again) that the calculation of per-operator juice reflects the proportion of tuples that the operator has processed with respect to the entire {source input}. To ensure this, the denominator $T_{o}^{i}$  is the total number of tuples {sent out} from an operator $o$'s $i^{th}$ parent  per unit time, not merely tuples received by $o$. 

%\ig{this statement/para is confusing and needs to be clarified.}

%\ig{Second example figure would be much more readable if you annotated the juice values as well (perhaps in a different color).}

%\ig{please double check all calculations.}
\noindent {\bf  Example 1: }  Consider Fig.~\ref{simple-topology} in Section~\ref{background}. $J_{A}^{s} = 1 \times \frac{10K} {10K} = 1$ and $J_{B}^{s} = J_{A}^{s} \times \frac{8K} {16K} = 0.5$. 
B has a $T_{B}^{A}$ of 16K and not 8K, since B only receives half the tuples that were sent out by operator A, and its per-operator juice should be in context of only this half (and not all source input).

The value of $J_{B}^{s}=0.5$ indicates that B processed only half the tuples sent out by parent A. This occurred as the parent's output was split among children. (If (alternately) B and C were sinks (if D were absent from the topology), then their  juice values would sum up to the topology's juice.). D has two parents: B and C. C is only able to process 6K as it is congested. Thus, $J_{C}^{s}= J_{A}^{s} \times \frac{6K} {16K}=0.375$. $T_{D}^{C}$ thus becomes 6K. Hence, $J_{D}^{C} = 0.375 \times \frac{6K} {6K} = 0.375$. $J_{D}^{B}$ is simply $0.5 \times \frac{8K} {8K} = 0.5$. We sum the two and obtain $J_{D}^{s} = 0.375 + 0.5 = 0.875$. It is less than 1.0 as C was unable to process all tuples due to  congestion.\\ %\ig{Please do not remove this newline. It is a break between the example and an important part of the algo.}

\noindent \textbf{Example 2 (Topology Juice with Split and Merge):} %\ig{If space is an issue, this example and its figure can be removed. }

\begin{figure}[h!]
\vspace{-0.3em}
\includegraphics[width=1\columnwidth]{figures/complex-topology.pdf}
%\end{center}
\vspace{-1.5em}
\caption{{\bf {Juice Calculation in a Split and Merge Topology.}} }% A more complex topology with juice = 0.475 (average of juice of sink bolts).}%\fkc{Fixed dropping annotation. Rename bolt to operator} %\ig{This caption is too close to its figure, and the figure is too close to text above it.}
\label{complicated-topology}
\vspace{-0.1cm}
\end{figure}


In Fig.~\ref{complicated-topology}, we show how our approach generalizes to: a) multiple sources (spout 1 \& 2), and b) operators splitting output (E to B and F) and c) operators with multiple input streams (A and E to B). Bolt A has a juice value of 0.5 as it can only process half the tuples spout 1 sent it. Bolt D has a juice value of 1.0. 50\% of the tuples from D to E are unprocessed due to congestion at E.  E passes its tuples on to B and F: both of them get half of the total tuples it sends out. Therefore, B has juice of 0.25 from E and 0.5 from A  ($0.25+0.5=0.75$). 20\% of the tuples E sent F are unprocessed at F as it is congested, so F has  a juice value of $0.25\times0.8=0.2$. C processes as many tuples as B sent it, so it has the same juice as B (0.75). The juice of the topology is the sum of the juices of the two sinks, normalized by the number of sources. Thus, the topology's juice is  $\frac{0.2+0.75}{2} = 0.475$.%\ig{B from B?}
%Then, B has juice of 0.5 from A and E has a juice value of 0.5 from D.


 


%Users can set a minimum expectation of a topology's juice at all times, and this suffices as their throughput SLO. This SLO can be used to define the topology's utility function. For example, the utility function~\ref{eq:5} in Section~\ref{utility} becomes:

%\small
%\begin{center}
%	\begin{equation} 
%	Utility = min(1, \frac{Current\ Juice}{Juice\ Threshold})  \times Job\_Max\_Utility
%%	 \textbf{this is min of 1, and frac}
%	\label{eq:juice}
%	\end{equation}

%\end{center}
%\vspace{-0.5em}
\normalsize


\noindent{\bf Some Observations:} First, while our description used unit time, our implementation calculates juice using a sliding window of 1 minute, collecting data in sub-windows of length 10 s. This needs only loose time synchronization across nodes (which may cause juice values to momentarily exceed 1, but does not affect our logic). Second, eq.~\ref{eq:2} treats all processed tuples equally--instead, a weighted sum could  be used to capture the higher importance of some sinks (e.g., sinks feeding into a dashboard). Third, processing guarantees (exactly, at least, at most once) are orthogonal to the juice metric. Our experiments use the non-acked version of Storm (at most once semantics), but Henge also works with the acked version of Storm (at least once semantics).

%e intervals time. This window should be neither too small nor too large. While our examples used unit time, this time interval length is configurable. A shorter interval implies that congestion can be detected quickly (and the scheduler can respond quickly), however it may trigger frequent re-allocations, e.g., upon spikes. A longer time interval may take longer to respond, but is resistant to spikes. In practice, we use a sliding window of measurements (at each operator), and calculate the juice within sub-windows. Our implementation uses a sliding window of 1 minute for data collection, and calculates the juice every 10 s (in sub-windows). %\igc{
	%Due to loose time synchronization juice values may momentarily exceed 1. 
	

%} %As we count the number of tuples entering and exiting an operator in the same time window for one calculation, we sometimes observe values of juice that are greater than 1. 

%\fkc{Here, we can add that this technique is for at-most once semantics. We can talk about how we can extend this to at-most once (in the acking mechanism). Is Spark Streaming, this should be easy -- as its not a continuous operator, only what is transmitted is computed.} \ig{a) Not sure. b) Not sure this is the right place to discuss this. Isn't juice measuring how close you are to exactly once semantics? 1.0 => exactly once (well, perhaps at least once).} \fkc{We cannot make any processing guarantees. For exactly once, we have to ensure somehow that each tuple that is input gets processed. All we do is make sure that the number of tuples that are processed per unit time is equal to the number of tuples that are input into the topology -- we do not know \emph{which} tuple it is that is getting processed. For placement, should we have a discussion section at the end where we discuss issues like processing guarantees and statefulness etc?} \ig{Let's not mention exactly/at least once in this section at all. There is some mention in the intro - PTAL. And then we can discuss in the Implementation section. That's all - only 2 occurrences. Don't overdiscuss it, as the paper is not about semantics.}

==> henge-arxiv 2/text/10-implementation.tex <==
\vspace{-0.1cm}
\section{Implementation}
\label{system-architecture}


We integrated Henge into Apache Storm~\cite{storm_web}. Henge involves 3800 lines of Java code. It is an implementation of the predefined IScheduler interface. The scheduler runs as part of the Storm Nimbus daemon, and  
%The developer can specify which scheduler to use in a configuration file that is provided to Nimbus.  
%The Storm scheduler 
is invoked by Nimbus periodically every 10 seconds. Further changes were made to Storm Config, allowing users to set topology SLOs and utility functions while writing topologies.

\begin{figure}[h!]
	\begin{center}
 	 \vspace{-0.3cm}
		\includegraphics[width=1\columnwidth]{figures/architecture.pdf}
	\end{center}
	\vspace{-0.5cm}
	\caption{{\bf Henge Implementation:} \it Architecture in Apache Storm.}
	\label{henge-architecture}
 	\vspace{-0.3cm}
\end{figure}

Henge's architecture is shown in Fig.~\ref{henge-architecture}. The Decision Maker implements the Henge state machine of Section \ref{policy}. The Statistics Module continuously calculates cluster and per-topology metrics such as the number of tuples processed by each task of an operator per topology, the end-to-end latency of tuples, and the CPU load per node. This information is used to produce useful metrics such as juice and utility, which are passed to the Decision Maker. The Decision Maker runs the state machine, and sends commands to Nimbus to implement actions. %\ig{Which component sends the commands to initiate actions? Decision Maker? Say so!}
The Statistics Module also tracks past states so that reversion can be performed. %also tracks  historical performance and configuration of topologies whenever a reconfiguration is performed by the Decision Maker, so that reversion can be performed. 


 
%\igc{The measurement of metrics such as juice and latency rely on close (but not accurate) synchronization of clocks across the cluster. We use NTP which has a typical error of 1 ms or so, and this suffices for us.}

%\ig{Are there other implementation notes like this one? } 

%\igc{

%\fkc{I will add and make cohesive 2) shuffle grouping } \ig{When? We need to do this now! Put it in some color font so I will see it clearly.} %at least once, and acking is discussed 1) statefulness
%\fkc{The goal of Henge is to reconfigure congested operators to improve SLO satisfaction. } 


%Henge can also handle stateful topologies that checkpoint their data in a central store (e.g., HDFS). 

% handles stateful operators by storing it in a central place (e.g., HDFS) before rebalancing/reconfiguration, and fetch after the step is done.
%}



%Notes from Bobby meeting -- (Kerberos relies on it). Time millis  has some strangeness, e.,g a leap second, or time goes back. Could replace our current latency mechanism with acks (so spout measures executiom time for tuple).}

==> henge-arxiv 2/text/11-eval-new.tex <==
\vspace{-0.1cm}
\section{Evaluation}
\label{evaluation}


%We evaluate the correlation of juice to other system-observed metrics, and benefits from the Henge policy.

We evaluate Henge with a variety of workloads, topologies, and SLOs. 

%\ig{use the term ``natural fluctuations" in this section when referring to such behavior in the plot (this term was created in the intro and needs some tangible references here to close the bracket). }


%\ig{Please watch font sizes. The font in this section seems too small (compared to the previous sections).}

\noindent\textbf{Experimental Setup:} By default, our experiments used the Emulab cluster~\cite{White+:osdi02}, with machines (2.4 GHz, 12 GB RAM) running Ubuntu 12.04 LTS, connected via a 1 Gbps connection. Another machine runs Zookeeper~\cite{zookeeper_web} and Nimbus. Workers (Java processes running executors) are allotted to each of our 10  machines (we evaluate scalability later). 

\begin{figure}[h!]
	\centering
		\vspace{-0.2cm}
	\includegraphics[width=1.0\columnwidth]{figures/topologies.pdf}
	\vspace{-0.6cm}
	\caption{\bf Three Microbenchmark Topologies.}
	\label{topology-types}
	\vspace{-0.5cm}
\end{figure}
\vspace{-0.1cm}
\begin{figure}[h!]
	\centering
	\includegraphics[width=1.0\columnwidth]{figures/pageload.pdf}
	\vspace{-0.6cm}
	\caption{\bf PageLoad Topology from Yahoo!.}
	\label{pageload}
	\vspace{-0.5cm}
\end{figure}

\noindent\textbf{Topologies: } For evaluation, we use both: a) micro-topologies that are possible sub-parts of larger topologies~\cite{xu:16:ic2e}, shown in Fig.~\ref{topology-types}; and b) a production topology from Yahoo! Inc.~\cite{xu:16:ic2e}--this topology is called ``PageLoad" (Fig.~\ref{pageload}).  Operators are the ones that are most commonly used in production: filtering, transformation, and aggregation. In each experimental run, we initially allow topologies to run for 900 s without interference (to stabilize and to observe their performance with vanilla Storm), and then enable Henge to take actions. All topology SLOs use the knee utility function of Section~\ref{job-utilities}. Hence, below we use ``SLO'' as a shorthand for the SLO threshold.




        
\begin{comment}

\begin{figure*}[t]
\begin{subfigure}{1\textwidth}
\centering
        \includegraphics[width=1\columnwidth]{figures/resources-vs-config.pdf}
        \vspace{-0.6cm}
        
        \caption{In each  plot, the x-axis represents the initial parallelism of an intermediate operator in a linear topology. The left y-axis shows the final parallelism level Henge assigned to the operator, and the right y-axis shows the number of rounds required to reach said parallelism level. From left to right, topologies have increasingly less strict SLOs to satisfy. The dashed black line passing through the final number of executors for certain configurations indicates that the final configuration is the same as the initial configuration and no reconfiguration was required.}
        \label{resources-used}
        \end{subfigure}
        \vspace{-0.1cm}
        \begin{subfigure}{1\textwidth}
                \centering
                \includegraphics[width=1\columnwidth]{figures/config-slo.pdf}
                \vspace{-0.6cm}
        \caption{Corresponding to the plots in Fig.~\ref{resources-used}, the y-axis shows the utility that can be achieved with each configuration. }
            \label{changing-congestion}
        \end{subfigure}
        \caption{}
        \vspace{-0.3cm}
        \end{figure*}
        
        
\begin{figure*}[t]
        \begin{subfigure}{1\textwidth}
                \centering
                
                \includegraphics[width=1\columnwidth]{figures/resources-vs-config.pdf}
                \vspace{-0.2cm}
                \caption{In each of the above plots, the x-axis represents the initial parallelism of a single intermediate operator in a linear topology. The left y-axis shows the final parallelism level Henge assigned to the operator, and the right y-axis shows the number of rounds required to reach said parallelism level. The dashed black line passing through the final number of executors for certain configurations indicates that the final configuration is the same as the initial configuration and no reconfiguration was required.}
                \label{resources-used}
        \end{subfigure}\\
        \vspace{-0.1cm}
        \begin{subfigure}{1\textwidth}
                \centering
                \includegraphics[width=1\columnwidth]{figures/config-slo.pdf}
                \vspace{-0.2cm}
        \caption{Corresponding to the plots in Fig.~\ref{resources-used}, the x-axis represents the initial parallelism of a single intermediate operator in a linear topology. The y-axis shows the utility that can be achieved with this configuration. From left to right, topologies have increasingly less strict SLOs to satisfy. Red circles show the utility achieved before Henge performs reconfiguration and blue circles show the utility achieved after reconfiguration. If no blue circles are present, no reconfiguration was required.\fkc{Reduce white space. Make scale equal so we can cut out the numbers and make the plots bigger} }
            \label{changing-congestion}
        \end{subfigure}
\caption{}
        
\end{figure*}
\end{comment}
% \vspace{-0.2cm}


\begin{comment} %deprecated
\begin{figure}[t]
	\vspace{-0.5cm}
	\begin{center}	
	\includegraphics[width=1\columnwidth]{figures/simple-convergence/exp81/all.pdf}
		\vspace{-0.5cm}
		\caption{Solid lines indicate reconfiguration for T2. As T2 is reconfigured, it meets its SLO and total utility of the cluster reaches its expected value (15). } 	\vspace{-0.2cm}
		\label{microbenchmark-slo}
		\vspace{-0.5cm}
	\end{center}
\end{figure}
\end{comment}

\input{text/11a-evaluation-juice}
\input{text/11b-evaluation-henge}




==> henge-arxiv 2/text/11a-evaluation-juice.tex <==
% \vspace{0.6cm}
\subsection{Juice as a Performance Indicator} %\fkc{exps here were done with 6 machines}
\label{juice-evaluation}

 \noindent{\bf Juice is an indicator of queue size: } Fig.~\ref{queue-size} shows the inverse correlation between topology juice and queue size at the most congested  operator of a PageLoad topology. Queues buffer incoming data for operator executors, and longer queues imply slower execution rate and higher latencies. Initially queue lengths are high and erratic--juice captures this by staying well below 1. At the reconfiguration point (910 s) the operator is given more executors, and juice converges to 1 as queue lengths fall, stabilizing by 1000 s. 
 
\vspace{-0.3cm}
\begin{figure}[h]
		\begin{center}
			\includegraphics[width=1.0\columnwidth]{figures/queueing-delay/all.pdf}
		\end{center}
	\vspace{-0.5cm}
	\caption{{\bf Juice vs. Queue Size:} \it Inverse Relationship.}
    \vspace{-0.1cm}
	\label{queue-size}
\end{figure}

%\begin{figure}

%\begin{center}
%\includegraphics[width=1\columnwidth]{figures/juice-figures/exp102-star-shape/figure.pdf}
% 	\vspace{-0.6cm}
%\caption{Juice remains stable at 1.0 (Star topology), even though input rate is 4 $\times$ as much as output rate.}
%\label {star-juice} \vspace{-0.5cm}
%\end{center}
%\end{figure} 

\begin{figure}
	\begin{center}
		\vspace{-0.1cm}
\includegraphics[width=1.0\columnwidth]{figures/juice-figures/exp95-juice/juice-line.pdf}\vspace{-0.2cm}
\caption{{\bf Juice is Rate-Independent:} \it Input rate is increased by 3 $\times$ at 4000 s, but juice does not change. When juice falls  to 0.992 at 4338 s, Henge  stabilizes it to 1.0 by 5734 s. }%\ig{make juice a line in this plot, not points. others can remain points.}
\vspace{-0.5cm}
\label {page-load-tuples} 
\end{center}
\end{figure}
 
 %Fig.~\ref{queue-size}  plots the executor queue sizes (tuples) in  a single operator of a PageLoad topology. Queues buffer incoming data for operator executors, and longer queues imply slower execution rate and higher latencies. %In Storm, each executor gets tuples for each of its tasks from this queue. 
 %Growth in queue length implies the operator's execution rate is slower than the input rate, leading to higher latency.  
 %The plot shows that juice and queue size are, as expected, inversely related: initially queue lengths are high and erratic at the same time as the juice is well below 1. At the reconfiguration point (at 910 s), juice starts to converge to 1 by 1000 s; concurrently queue lengths fall and stabilize. %as juice improves (at the reconfiguration point), the queue size falls. As juice converges to 1.0 (\ig{at time t=??}), the queue size has also fallen and  stabilized. %, meaning that the processing rate is able to keep up with input rate.

%\ig{Don't use bolt and operator in the same section. Or, if you do, please specify clearly that we use them interchangeably.}%stated earlier on

%To be truly general, juice must remain a number between $[0,1]$ even as the topology shape, input rate and functions change. 

%\noindent{\bf Juice is independent of topology, input rate, and operators: } %Fig.~\ref{star-juice}  shows (for an uncongested star-shaped topology that has 4 spouts, 4 sinks and 1 intermediate center operator) that juice is 1.0, instead of 4.0 (which might be expected due to 4 sources). This shows juice is  independent of the number of spouts and sinks, illustrating  point (2) above.

%The topology is tuned to ensure that none of the operators is congested. 
%As juice is independent of the shape of the topology, it always remains 1.0.  If it was not topology independent, juice would be proportional to the number of sources (equal to 4.0 instead of 1.0).

\noindent{\bf Juice is independent of operations and input rate: } In Fig.~\ref{page-load-tuples}, we run 5 PageLoad topologies on one cluster, and show data for one of them. Initially juice stabilizes to around 1.0, near t=1000 s (values above 1 are due to synchronization errors, but they don't affect our logic). PageLoad filters tuples, thus output rate is $<$ input rate--however, juice is 1.0 as it shows that all input tuples are being processed.

Then at 4000 s, we triple the input rate to all tenant topologies. Notice that juice stays 1.0. Due to natural fluctuations, at 4338 s, PageLoad's juice drops to 0.992. This triggers  reconfigurations (vertical lines) from Henge, stabilizing the system by 5734 s, maximizing cluster utility.

%we show that juice is independent of operator type as well as the input rate of the topology.  In  Fig.~\ref{page-load-tuples}, we show results from one PageLoad topology that is running on a cluster with 4 other topologies. Up until 4000 s, the topologies runs with a constant input rate. At 1000 s, Henge performs resource reallocation so the topology shown is able to keep up with the input rate and juice becomes 1.0. If juice was dependent on the function of operators, it would be proportionate to the number tuples that are filtered out and aggregated.  At 4000 s, the input rate increases by 3$\times$ for all tenants. Juice drops to 0.992 for the shown topology, which triggers a rebalance. After resource reallocation, the topology is able to keep up with the input rate. Juice becomes 1.0 at 5743 s, instead of increasing in proportion to the input rate. \ig{I had a comment here. You will have to explain why juice goes above 1.0.} 


==> henge-arxiv 2/text/11b-evaluation-henge.tex <==
\subsection{Henge Policy and Scheduling} 
\label{policy-evaluation}

\subsubsection{Impact of Initial Configuration}%\hfill
\begin{figure}[h!]
	\begin{center}
	\vspace{-0.2cm}
\includegraphics[width=1.0\columnwidth]{figures/capacity-vs-init-config-.pdf}%capacity-vs-init-config-.pdf
\vspace{-0.3cm}
\caption{{\bf Performance vs. Resources in Apache Storm:} \it The x-axis shows initial parallelism of one intermediate operator in a linear topology. Left y-axis shows initial capacity of the operator. Right y-axis shows stable utility  reached without using Henge.} % for a topology with an operator of that parallelism.
%Multiple instances of the same topology are run with latency SLOs that vary from stringent (40 ms) to relaxed (60 ms).  }%\fkc{referring to 70 ms data for now, will add back the plots later}
		\label{changing-capacity}
	\end{center}
\vspace{-0.5cm}
\end{figure}


\begin{figure}[t]
\vspace{-0.8cm}%From box/../config/*
        \centering
        %\includegraphics[width=1\columnwidth]{figures/capacity-variation-bars-4.pdf}%capacity-variation-bar.pdf%Presentation.pdf/capacity-variation-bars-3.pdf
        \includegraphics[width=1\columnwidth]{figures/init-config/init-config-vs-slo-resources.pdf}
        \vspace{-0.5cm}
\caption{{\bf Effect of Henge on Figure~\ref{changing-capacity}'s initial configurations:} %The x-axis is initial parallelism of an intermediate operator in a linear topology. 
\it SLOs become more stringent from bottom to top. We also explore a 2  $\times$ higher input rate. a) Left y-axis shows final parallelism level Henge assigned to each operator. Right y-axis shows number of rounds required to reach said parallelism level. b) Utility values achieved before and after Henge. }%The y-axis shows the utility that can be achieved with each initial configuration, and the utility that can be achieved after Henge performs reconfiguration. }%\fkc{convert to bar plot}\fkc{referring to 70 ms data for now, will add back the plots later}
    \label{changing-congestion}
\vspace{-0.4cm}
\end{figure}


%\ig{this plot has squished right y axis - change labels to 5, 15, 25, 35. } done
\noindent{\bf State Space: }  Fig.~\ref{changing-capacity} illustrates the state space that Henge needs to navigate. These are runs {\it without} involving Henge. We vary the initial number of executors for an intermediate operator. Fewer initial executors   (5, 10) lead to a high capacity (indicating congestion: Section~\ref{congestion}) and consequently the topology is  unable to achieve its SLO. From the plot, the more stringent the SLO, the greater the number of executors needed to reach max utility. Except very stringent jobs SLOs (40, 50 ms) all others can meet their SLO. %, even though no resource bottlenecks exist.  %)\ig{give section number where definition of capacity appears}
%~\ref{resources-used} and
%\noindent\textbf

%We first illustrate the state space that Henge needs to navigate. Fig.~\ref{changing-capacity} shows the effect of initial state  on a linear topology, {\it without} involving Henge. We vary the initial number of executors for an intermediate operator. Fewer initial executors   (5, 10) lead to a high capacity (indicating congestion: Section~\ref{congestion}) and consequently the topology is  unable to achieve its SLO. From the plot, the more stringent the SLO, the greater the number of executors needed to reach max utility. Only topologies with very stringent latency SLOs (40, 50 ms) never meet their SLO. %, even though no resource bottlenecks exist.  %)\ig{give section number where definition of capacity appears}
%~\ref{resources-used} and
%\noindent\textbf



\noindent{\bf Henge In Action: } Now, we put Henge into action on  Fig.~\ref{changing-capacity}'s topology and initial state, with max utility 35. Fig.~\ref{changing-congestion} shows the effect of varying: a) initial number of executors (5 to 25), b) latency SLO (40 ms to 60 ms), and  c)  input rate. We plot converged utility, rounds needed, and executors assigned. %The plot shows the converged utility achieved by Henge, along with the number of rounds needed and executors assigned by it.  %show the utility a topology can provide and the resources required to provide said utility. We use the same linear topology as Fig.~\ref{changing-capacity}, and set its max utility value to 35. %Henge is allowed to perform reconfiguration to improve system utility. 
 
 We observe that generally, Henge gives more resources to topologies with more stringent  SLOs and  higher  input rates. For instance, for a congested operator initially assigned 10 executors in a 70 ms SLO topology, Henge  reconfigures it to have an average of 18 executors, all in a single round. On the other hand, for a stricter 60 ms SLO it assigns 21 executors in two rounds. % the number of executors finally assigned to an operator with the same initial configuration, belonging to a topology with an SLO of 60 ms is 21, assigned in two rounds. However, 
 When we double the input rate of these two topologies, the former is assigned 36 executors in two rounds and the latter is assigned 44, in 5 rounds.  % actually, average values are 18.5, 21.5 (better floor than round?)  %\ig{For example, ... talk about one experiment on the plot, how much resources it needs to meet SLOs, and how long it takes -- make it concrete!...} dynamic
 
 
 
 
 %to allow topologies to satisfy their SLO, even though we observe from the plot that 100\% utility (or 100\% SLO satisfaction) is never achieved.  
 

 
 %\fkc{The corresponding utility plot in 13b is there to show that the 40 and 50 ms SLOs are both difficult to meet (given all other factors), with respect to this paragraph. However, I can still take it out. }
 
 
 

Henge convergence is fast. In Fig.~\ref{changing-congestion}a, convergence occurs within 2 rounds for a topology with a 60 ms  SLO. Convergence time increases for stringent SLOs and higher input rates. With the 2 $\times$ higher input rate convergence time is 12 rounds for stringent SLOs of 50 ms, vs. 7 rounds for 60 ms.

Henge always reaches  max utility (Fig.~\ref{changing-congestion}b) unless the SLO is unachievable (40, 50 ms SLOs). % As long as CPU is the bottleneck, Henge always converges. 
Since Henge aims to be minimally invasive, we do not explore operator migration (but we could use them orthogonally~\cite{twochoices,morethantwochoices,network-aware-placement}).%   operators. Migration techniques can be combined with Henge to further improve SLO satisfaction~\cite{twochoices,morethantwochoices,network-aware-placement}. 

%We note an interesting pattern in Henge's behavior when the SLO is not achievable (40 and 50 ms). 
 With an SLO of 40 ms, Henge actually performs fewer reconfigurations and allocates less resources than with a laxer SLO of 50 ms. This is because the 40 ms topology gets black-listed earlier than the 50 ms topology ( Section~\ref{reversion}: recall this occurs if utility improves $<$ 5\% in a round). %When Henge notices that allocating resources to a topology with an SLO of 40 ms does not improve the topology utility by at least 5\% per round, it black-lists the topology and does not give it additional resources. On the other hand, for topologies with a more achievable SLO, e.g., 50 ms, it tries for longer (though it never meets the SLO threshold). This behavior is expected for hard-to-achieve SLOs. 

Overall, by black-listing  topologies with overly stringent SLOs and satisfying other topologies, Henge meets its goal of preventing resource hogging  (Section~\ref{summary}).%due to stringent SLOs

%These results show that in our setting, latency SLOs of 50 ms and below are unachievable. Therefore, in all further experiments, we set higher latency SLOs. %\fkc{check and add all latency SLOs.}
%if efficient migration techniques are invented in the future for stream processing systems, they can be combined with Henge to further improve SLO satisfaction.

%\fkc{Based on our deep dive we found that -- seems intuitive. Plus, this is the problem we set out to solve.}


 
\subsubsection{Meeting SLOs}


%\ig{Please italicize every figure caption (after the bold fonted heading), like I've done in Figure~\ref{discussion:mixed-topologies}. Will help distinguish captions from text. Otherwise, these pages are very monotonous to visualize.}

%\ig{I don't even know which figure this one is referring to (no figure is referenced), or how you show that the highest priority topology is picked. perhaps we can annotate the plot?} 
%\ig{what kind of topology?}

\noindent{\bf Maximizing Cluster Utility: } To maximize  total cluster utility, Henge greedily prefers to reconfigure those topologies first which have a higher max achievable utility (among those missing their SLOs). In Fig.~\ref{discussion:mixed-topologies}, we run 9 PageLoad topologies on a cluster, with max utility values ranging from 10 to 90 in steps of 10. The SLO threshold for all topologies is 60 ms.  %We prevent Henge from performing reconfiguration within the first 900 seconds. 
Henge first picks T9 (highest max utility of 90),  leading to a sharp increase in total cluster utility at 950 s. Thereafter, it continues in this greedy way.  We observe some latent peaks when topologies reconfigured in the past stabilize to their max utility. For instance, at 1425 s we observe a sharp increase in the slope (solid) line as T4 (reconfigured at 1331 s) reaches its SLO threshold.  All topologies  meet their SLO within 15 minutes (900 s to 1800 s). %Hence Henge maximizes total cluster utility.

\begin{figure}[h!]
	\vspace{-0.1cm}	% in mixed-utilities exp
	\begin{center}
\includegraphics[width=1.0\columnwidth]{figures/mixed-utilities/mixed-utilities.pdf} 
\vspace{-0.7cm}
\caption{{\bf Maximizing Cluster Utility:} \emph{Red (dotted) line is total system utility. Blue (solid) line is magnified slope of the red line. Vertical lines are reconfigurations annotated by the job touched. Henge reconfigures higher max-utility jobs first, leading to faster increase in system utility.}} %
		\label{discussion:mixed-topologies}
	\end{center}
\vspace{-0.25cm}
\end{figure}




\noindent{\bf Hybrid SLOs:} We evaluate a hybrid SLO that has separate thresholds for latency and juice, and two corresponding utility functions (Section~\ref{job-utilities}) with identical max utility values. The job's utility is then the average of these two utilities. %\fkc{Add that users can give different weights to different types of SLOs, instead of half-half.}

Fig.~\ref{cluster-intrusive} shows 10 (identical) PageLoad topologies with hybrid SLOs running on a cluster of 10 machines. Each topology has SLO thresholds of: juice 1.0, and latency 70 ms.  The max utility value of each topology is 35. Henge only takes about 13 minutes (t=920 s to t=1710 s) to reconfigure all topologies successfully to meet their SLOs.  9 out of 10 topologies required a single reconfiguration, and one (T9) required 3 reconfigurations. %, shown on the plot.% (\ig{give the times}). %the times alone give little meaning 
%\vspace{-0.7cm}	\ig{what kind of topology?}


\begin{figure}[h!]
	\begin{center}%exp161
	\vspace{-0.2cm}
\includegraphics[width=1.0\columnwidth]{figures/hybrid-utilities/hybrid-new.pdf} %exp161
\vspace{-0.7cm}
\caption{{\bf Hybrid SLOs: } \it Henge Reconfiguration.}%\ig{no}.\fkc{do we need to explain the initial bump at 200s? It's due to the fact that when the topology pipeline isn't full and tuples haven't come out of the sink, we record the latency values as 0 which means perfect SLO satisfaction according to the utility function} }%\ig{1) Add a horizontal line showing the max total utility (do this for all plots where you show the total cluster utility). 2) Make the sum a line, not a collection of points. There is no need to show the mean. }
		\label{cluster-intrusive}
	\end{center}
\vspace{-0.5cm}
\end{figure}


% \noindent\textbf{Stateful Topology} 
% \fkc{This is going to have some overhead. Skip?} \ig{Can be lower priority and not needed for first draft. But since you will have time in April we should do this plot!}

%\ig{when compiled without comments, figures bunch up a lot. please fix.}

%\ig{all captions must end in periods (.) E.g., Fig 16 (check all others).}

\subsubsection{Handling Dynamic Workloads} 



%\ig{this is too long to be a subsubsection. should be at least a subsection.}

%\ig{Seems like it's the other way around. what is B's spike? Also this plot is indistinguishable in black and white.}

\noindent{\bf A. Spikes in Workload:} 
Fig.~\ref{discussion:step-workload} shows the effect of a workload spike in Henge. Two different PageLoad  topologies A and B are subjected to input spikes. B's  workload spikes by 2 $\times$, starting from 3600 s. The spike lasts until  7200 s when A's spike (also 2 $\times$) begins.   Each topology's SLO is 80 ms with max utility is 35. Fig.~\ref{discussion:step-workload} shows that: i)  output rates keep up for both topologies both during and after the spikes, and ii) the utility stays maxed-out  during the spikes. In effect, Henge completely hides the effect of the input rate spike from the user. 
%} \ig{swap orders of a and b figures, and give them names a and b.}



% \begin{figure}[h]
% \vspace{-0.1cm}
% \begin{subfigure}{0.5\textwidth}
%                 \centering
%                 \includegraphics[width=1\columnwidth]{figures/discussion-figures/stepping-workload/output-tuples.pdf}\vspace{-0.2cm}
%         \caption{Variation in workload as time progresses.}\vspace{-0.1cm}
%             \label{discussion:step-workload-a}
%         \end{subfigure}
%         \vspace{-0.1cm}
%         \begin{subfigure}{0.5\textwidth}
%                 \centering
%                 \includegraphics[width=1\columnwidth]{figures/discussion-figures/stepping-workload/output-utilities.pdf}\vspace{-0.2cm}
%         \caption{The sum utilities of the topologies on the cluster.}\vspace{-0.3cm}
%             \label{discussion:step-workload-b}
%         \end{subfigure}
% \caption{Spikes in Workload.}
% 		\label{discussion:step-workload}
	
% \vspace{-0.3cm}
% \end{figure}

%\ig{Please be consistent in your labels! E.g., some plots y axes labels are Sum of Utility, others are Utility Sum. There are others.}


\begin{figure}[h]
\vspace{-0.1cm}

                \centering
                \includegraphics[width=1\columnwidth]{figures/discussion-figures/stepping-workload/output+tuples+annotated.pdf}\vspace{-0.2cm}
        \caption{{\bf Spikes in Workload:} \it Left y-axis shows total cluster utility (max possible is $35\times 2=70$). Right y-axis shows the variation in workload as time progresses.}\vspace{-0.1cm}
		\label{discussion:step-workload}
	
\vspace{-0.3cm}
\end{figure}

	\begin{figure}[h!]
	\begin{center}
% \includegraphics[width=1.0\columnwidth]{figures/diurnal-v2/diurnalcombined-with-storm-configured.pdf}
\includegraphics[width=1.0\columnwidth]{figures/diurnal-v2/diurnal-no-sdsc.pdf}
\vspace{-0.8cm}

% \caption{{\bf Diurnal Workload:} \it a) Input and output rates  over time, for two different diurnal workloads. b) Utility of a topology (reconfigured by Henge at runtime) with the SDSC workload, and c) with the EPA workload, d) CDF of SLO satisfaction for Henge, default Storm, and manually configured. Henge adapts during the first cycle and fewer reconfigurations are required thereafter. %Henge adapts durin gthe first day itself and does not need During the first cycle (day), Henge adapts all topology configurations to the workload. Subsequent cycles need fewer reconfigurations. \
% }

\caption{{\bf Diurnal Workload:} \it a) Input and output rates  over time, for two different diurnal workloads. b) Utility of a topology (reconfigured by Henge at runtime) with the EPA workload, c) CDF of SLO satisfaction for Henge, default Storm, and manually configured. Henge adapts during the first cycle and fewer reconfigurations are required thereafter. }

%\fkc{(change (d) to percentage on the x-axis.) Should we keep d as a timeline of all runs (vanilla, manual and Henge) because I discuss the percentiles in the text anyway?} \ig{d is ok. let's keep it. this is not the time to plot, but to doublecheck everything. The vspace below this caption is awful.}
		\label{diurnal}
	\end{center}
\vspace{-0.8cm}
\end{figure}


\begin{comment}
henge:
117.307005126 | 5%
262.219546884 | 15
346.948395734 | 50
350.0 | 90 
350.0 | 95
350.0 | 99
308.410219562 | mean

default:
0.000963656295034
0.00109596540251
0.00231241799139
108.150164657
134.157105959
163.973222399
15.9573584939


configured
200.599639579
232.790448821
349.389546676
350.0
350.0
350.0
307.206293532
\end{comment}

% \vspace{0.2cm}
\noindent{\bf B. Diurnal Workloads:} Diurnal workloads are common for stream processing in production, e.g., in e-commerce websites~\cite{decandia2007dynamo} and social media~\cite{naaman2012study}.  %We evaluate how quickly Henge responds to a diurnal variation of input rate.  
We generated a  diurnal workload based on the distribution of the SDSC-HTTP ~\cite{web-trace1} and EPA-HTTP traces~\cite{web-trace2}, injecting them into PageLoad topologies.  
%The first trace contains a day's worth of all HTTP requests to the SDSC WWW server located at the San Diego Supercomputer Center in San Diego, California while the second contains a full day's worth of all HTTP requests to the EPA WWW server located at Research Triangle Park, NC.  
%We changed the workload of the PageLoad topology to reflect these distributions.  
5 topologies are run with the SDSC-HTTP trace and concurrently, 5 other topologies are run with the EPA-HTTP trace. All 10 topologies have max-utility=10 (max achievable cluster utility=350), and a latency SLO of 60 ms.  %\igc{Each topology has a max utility set to ??} %To speed up our experiment we mapped each hour of the trace to a 10-minute interval. We run  48 hours of the original trace.
% (8000 s)


Fig.~\ref{diurnal} shows the results of running 48 hours of the trace (each hour mapped to 10 min intervals). In Fig.~\ref{diurnal}a  workloads increase from hour 7 of the day, reach their peak by  hour 13$\frac{1}{3}$, and then start to fall. Within the first half of Day 1, Henge successfully reconfigures  all 10 topologies, reaching by hour 15 a cluster utility that is 89\% of the max. %(not shown)

Fig.~\ref{diurnal}b shows a topology running  the EPA workload (other topologies exhibited the same behavior). Observe how Henge reconfigurations from hour 8 to 16  adapt to the fast changing workload. This also results in fewer SLO violations during the second peak  (hours 32 to 40). Thus, even without adding resources, Henge tackles diurnal workloads. %Therefore, Henge is able to stabilize the cluster with minimal number of reconfigurations.  

% when Henge and default Storm are able to satusfy the SLO


%Fig.~\ref{diurnal}d compares the percentage of time during the run when Henge and default Storm are able to provide SLO satisfaction. 
Fig.~\ref{diurnal}c shows the CDF of SLO satisfation for the three systems. Default Storm performs  poorly, giving 0.0006\% SLO satisfaction at the median, and 30.9\% at the 90th percentile. ({This means that 90\% of the time, default Storm provided a total of at most 30.9\% of the cluster's max achievable utility.}) Henge yields 74.9\% , 99.1\%,  and 100\% SLO satisfaction at the 15th, 50th, and 90th percentiles respectively. 

Henge is also better than manual configurations. We manually configured all topologies to meet their SLOs at  median load. 
%In addition, we compare Henge's results to the utility provided by a cluster running topologies that are manually configured to achieve their SLO at the median load. To manually configure the topologies, we settle on the configuration Henge chose at the median load. Interestingly, the 
These provide 66.5\%, 99.8\% and 100\% SLO satisfaction at the 15th, 50th and 90th percentiles respectively. Henge is better than manual configurations from the 15th to 45th percentile, and comparable from then onwards. %This is because it is able to adapt to not only the median but also the peak workload. % Henge is better than manual configurations 85\% of the time (crossover  point). 

%We average the total cluster utility that Henge, default Storm, and manually configured topologies provide throughout the run of the experiment. 
Henge has an average of 88.12\% SLO satisfaction rate, whereas default Storm and manually configured topologies provide an average of  4.56\% and 87.77\% respectively. Thus, Henge provides 19.3 $\times$  better SLO satisfaction than default Storm, and performs better than manual configuration.%manually configured topology. % and avoids the overhead of manually configuring topologies to match the varying workload. %\ig{no idea where this 19.3 came from. please explain.}
%henge
%308.410219562


%default

%15.9573584939


%configured

%307.206293532


%At the 15th percentile, Henge performs significantly better; 
%85\% of the time, the SLO satisfaction provided by Henge does not fall below 74.9\%. \ig{repetitive, already mentioned.} %This is because Henge can adaptively reconfigure topologies to accommodate increases in workload; although this incurs an overhead at run-time, it ensures a degree of predictability in the SLO satisfaction of topologies. 
%The cost of Henge reconfigurations is evinced at the median: the manually configured topologies perform marginally better as they do not have to be reconfigured dynamically. \ig{this is really not visible and we should not talk about it.}


%\fkc{running experiment manually tuned for low latency with median workload}

%\ig{For Fig~\ref{diurnal} can we also compare against base storm (set to meet, e.g., median or average tuples per sec?). From 591IG seminar 3/31.} \fkc{that would require changing the initial configuration. we keep the same initial config for comparison}

\subsection{Production Workloads}  %\ig{changed to subsection to highlight good result.}
%\noindent{\bf C. Production Workloads:} %We evaluate the performance of Henge with tenant topologies on a cluster where each tenant has a high, varying  workload. \ig{what kind of?}


We configured the sizes of 5  PageLoad topologies based on data from a Yahoo! Storm production cluster and Twitter datasets~\cite{apollo-datasets}, shown in Table~\ref{table:yahoo-job-dist}. We use 20 nodes each with 14 worker processes. For each topology, we inject an input rate proportional to its number of workers. T1-T4 run sentiment analysis on Twitter workloads from 2011~\cite{apollo-datasets}. T5 processes logs at a constant rate. Each topology has a latency SLO threshold of 60 ms and max utility value of 35. %We show the results in Fig.~\ref{prod}.

% \igc{To further stress Henge, we underprovisioned the cluster so that not all SLOs could be met.} 

%exp237
\begin{comment}
31823.954
31894.028
31966.106
32042.074
32111.291
32184.322
32184.324
32184.327
32184.329
32184.331

% utility drops from 122.64090742132917  to 116.28488500805743. This a 5.182628330884588 drop
\end{comment}


% \vspace{-0.2cm}
\begin{table}[ht]% Try here, and then top
\begin{center}
\small
% \vspace{-0.2cm}
 \begin{tabular}{c c c c} 
 \toprule
Job & Workload & Workers & Tasks  \\ \hline
 T1 & Analysis (Egypt Unrest) & 234 & 1729 \\ \hline
 T2 & Analysis (London Riots)  & 31 & 459 \\\hline
 T3 &  Analysis (Tsunami in Japan)  & 8 & 100 \\\hline
 T4 &  Analysis (Hurricane Irene) & 2 & 34 \\\hline
 T5 &  Processing Topology & 1 & 18  \\ \bottomrule
 %1		2		8		31			234
 %18		33.5		100		459		
 %\label{yahoo-job-dist} 
\end{tabular}
\end{center}
\vspace{-0.5cm}
\caption{{\bf Job and Workload Distributions in Experiments: } \it Derived from Yahoo! production clusters, using Twitter Datatsets for T1-T4. (Experiments in Figure~\ref{prod}.)}%A worker is a JVM process that runs one or more tasks from operators in a topology.
\label{table:yahoo-job-dist}
\vspace{-0.3cm}
\end{table}
\normalsize 


\begin{figure}[h!]%exp237
\vspace{-0.2cm}	
	\begin{subfigure}{0.45\textwidth}
                \centering
                \includegraphics[width=1.0\columnwidth]{figures/production-workloads/cdf.pdf}\vspace{-0.3cm}
        \caption{\it CDF of the fraction of total time  tenant topologies provide a given SLO satisfaction. Max utility for each topology is 35.}%\vspace{-0.1cm}
            \label{prod-a}%\ig{total? initial?}
        \end{subfigure}
        \begin{subfigure}{0.45\textwidth}
                \centering
                \includegraphics[width=1.0\columnwidth]{figures/production-workloads/reversion-example_.pdf}\vspace{-0.1cm}
        \caption{\it Reconfiguration at 32111 s causes a drop in total system utility. Henge reverts the configuration of all tenants to that of 32042 s. Vertical lines show Henge actions for particular jobs.}\vspace{-0.2cm}
            \label{prod-b}
        \end{subfigure}\vspace{-0.05cm}
    		\caption{\bf Henge on Production Workloads.}%: 5 topologies running workloads from Yahoo! Storm production cluster and Twitter datasets~\cite{apollo-datasets}.
		\label{prod}
 \vspace{-0.1cm}
\end{figure}


This is an extremely  constrained cluster where not all SLOs can be met. Yet, Henge maximizes cluster utility. Fig.~\ref{prod-a} shows the CDF of the fraction of time each topology provided a given utility (including the initial 900 s where Henge is held back). T5 shows the most improvement (at the 5th percentile, it has 100\% SLO satisfaction), whereas T4 shows the worst performance (at the median, its utility is 24, which is 68.57\% of 35). %\ig{removed, as it sounds negative.}Henge is unable to scale out  T4 because it is small and the number of executors cannot exceed the number of tasks. %, which are limited according to the job distribution size. If more tasks were assigned to the operator, Henge could have scaled the operator out. 
The median SLO satisfaction for T1-T3 ranges from 27.0 to 32.3  (77.3\% and 92.2\% respectively). %T1 and T2 have highly varying workload and the workload of T3 is consistently very high. %Thus given equal priorities, larger workloads are prioritized by Henge. 


\noindent{\bf Reversion: } Fig.~\ref{prod-b} depicts Henge's reversion. At 31710 s, the system utility drops due to natural system fluctuations. This forces Henge to perform reconfigurations for two topologies (T1, T4). Since  system utility continues to drop, Henge is forced to reduce a topology (T5, which satisfies its SLO before and after reduction. As utility improves at 32042 s, Henge proceeds to reconfigure other topologies. However, the last reconfiguration causes another  drop in utility (at 32150 s). Henge reverts to the configuration that had the highest utility (at 32090 s). After this point, total cluster utility stabilizes at 120 (68.6\% of max utility). Thus, even under scenarios where Henge is unable to reach the max system utility it behaves gracefully, does not thrash, and converges quickly.%}\igc{\igc{along with a congested cluster (CPU load $>$ number of cores, at a majority of machines)} --> this is not true. A reversion occurred because there was a drop in utility, meaning that the last decision was unwise.






\subsubsection{Reacting to Natural Fluctuations}

% \begin{comment}
\begin{figure}[h!] %exp180
	\vspace{-0.4cm}
	\begin{center}
\includegraphics[width=1.0\columnwidth]{figures/reduction/reduction.pdf}\vspace{-0.3cm}
\caption{{\bf Handling CPU Load Spikes:} \it a) Total cluster utility. %Vertical black lines indicate Henge actions (reconfigurations and reductions). 
b) Average CPU load on machines in the CPU spike interval.}
		\label{reduction-plot}
	\end{center}
\vspace{-0.5cm}
\end{figure}

Natural fluctuations occur in the cluster due to  load variation that arises from interfering processes, disk IO, page swaps, etc. Fig.~\ref{reduction-plot} shows such a scenario. We run 8 PageLoad topologies, 7 of which have an SLO of 70 ms, and the 8th SLO is 10 ms. Henge resolves congestion initially and stabilizes the cluster by 1000 s. At 21800 s, CPU load increases sharply due to OS behaviors (beyond Henge's control). Seeing the significant drop in cluster utility, Henge reduces two of the topologies (from among those meeting their SLOs). This allows other topologies to recover within 20 minutes (by 23000 s). Henge converges the system to the same total utility as before the CPU spike.


\subsection{Stateful Topologies} 
\label{sec:stateful_expts}
 


%Henge's goal is to discover and resolve congestion in operators so topologies can meet their SLOs. 

% did another run after meeting


\begin{table}[ht]% Try here, and then top
\begin{center}
\vspace{-0.3cm}
 \small
 \begin{tabular}{ccc} %exp46
 \toprule
Job Type & Avg. Reconfig.   & Average  Convergence \\ 
 & Rounds (Stdev) & Time (Stdev) \\ \hline
 Stateful & 5.5 (0.58) &  1358.7355 (58.1s) \\ \hline
 Stateless & 4 (0.82) &  1134.2235 (210.5s)  \\\bottomrule
\end{tabular}
\end{center}
\vspace{-0.3cm}
\caption{{\bf Stateful Topologies:} \it Convergence Rounds and Times for a cluster with Stateful and Stateless Topologies.} %exp46 %\ig{this vspace is ugly. no space around captions. }
\label{table:stateful-properties}
\end{table}
\vspace{-0.2cm}
\normalsize

Henge handles stateful topologies gracefully,  alongside stateless ones. We ran four WordCount topologies with identical workload and configuration as T2 in Table~\ref{table:yahoo-job-dist}. Two of these topologies periodically checkpoint state to Redis (making them stateful) and have 240 ms latency SLOs. The other two topologies do not persist state in an external store and  have lower SLOs of  60 ms. Initially, none of the four meet their SLOs. Table~\ref{table:stateful-properties} shows results after convergence. Stateful topologies take 1.5 extra reconfigurations to converge to their SLO, and only 19.8\%  more reconfiguration time. This difference is due to external state checkpointing and recovery mechanisms, orthogonal to Henge.

%he other two stateless topologies have 60 ms SLOs -- > 

%Henge can reconfigure stateful topologies to meet their SLOs as long as they have an independent mechanism to recover state. This is because Henge relies on Storm's reconfiguration operation that restarts executors, causing them to lose state. The state recovery mechanism is orthogonal to Henge and can be checkpointing e.g., as in SEEP~\cite{seep}.

%We compare the convergence times for a stateful topology with one that is not. We configure two topologies with at-most once semantics that perform WordCount to have the same configuration and input workload as T2 in Table~\ref{table:yahoo-job-dist}. However, one topology regularly checkpoints state to Redis. We account for the checkpointing overhead and set the  topology's latency SLO to 240 ms. The other topology maintains the count in memory and has a latency SLO of 60 ms.  Table~\ref{table:stateful-properties} compares their convergence times when run on a 20 node cluster. The stateful topology takes 19.8\% longer to converge as the checkpointing overhead causes more congestion in its operators, which takes Henge more reconfiguration rounds to resolve. 



\subsection{Scalability and Fault-tolerance}

\label{scale_ft}
%We increase the number of topologies and cluster size, and inject failures during reconfiguration.

We vary number of jobs and nodes, and inject failures.


\subsubsection{Scalability}


\noindent{\bf Increasing the Number of Topologies:} Fig.~\ref{stepping-utility} stresses Henge by overloading the cluster with  topologies over time. We start with a cluster of 5 PageLoad topologies, each with a latency SLO of 70 ms, and max utility value of 35.  Every 2 hours, we add 20 more  PageLoad topologies. %, to observe if the additional load negatively impacts the pre-existing topologies and how Henge reconfigures all tenants to allow them to meet their SLO. %Fig.~\ref{stepping-utility-a} shows the average utility of tenant topologies at a particular time instance, and Fig.~\ref{stepping-utility-b} shows the number of reconfigurations the original tenants and the new tenants undergo when new topologies are added to the cluster.  %this is in the caption already

\begin{figure}[h!]  %updating to exp240
\vspace{-0.2cm}
	\begin{center}
% figures/increasing-topologies/exp236-re-run.pdf}
% %figures/stepping-utility.pdf
	\begin{subfigure}{0.5\textwidth}
                \includegraphics[width=1\columnwidth]{figures/increasing-topologies/max-utility.pdf}
        \caption{\it Green (dotted) line is average job utility. Blue (solid) line is number of job on  cluster. Vertical black lines are reconfigurations. %\fkc{should we remove the rebalance lines?}
        }\vspace{0.1cm}
            \label{stepping-utility-a}
        \end{subfigure}
    \begin{subfigure}{0.5\textwidth}
                \includegraphics[width=1.0\columnwidth]{figures/increasing-topologies/reconfigurations.pdf}%igurations
                \vspace{-0.2cm}
        \caption{\it Average number of reconfigurations that must take place when new topologies are added to the cluster.} 
            \label{stepping-utility-b}
        \end{subfigure}
        \vspace{-0.3cm}
		\caption{{\bf Scalability w.r.t. No. of Topologies: } \it  Cluster has 5 tenants. 20 tenants are added every 2 hours until the 8 hour mark. 
		 }%\fkc{Measure intrusiveness when more topologies are added}
		 %\ig{The labels in (b) seem botched, especially first two. Also this plot is neither referenced nor discussed.} %not sure what this means
		\label{stepping-utility}
	\end{center}
\vspace{-0.3cm}
\end{figure}
    
%\ig{ Can we draw a companion plot with this where y axis is the number of times reconfiguration occurred (total) until convergence vs. x axis is cluster size (you'd have 5, 115, 25, 25, 45)?}\fkc{cluster size is constant. This experiment is not scaled on increasing number of machines like Fig.21}

%\ig{can you draw the cdf of achieved utility (across all tenants) for each of the segments a-e? You'd have 5 lines one for each of a-e. this plot is interesting only if the CDF is not straight vertical line.} %\fkc{With the current data, the CDF would be a straight line. There was a different plot placed here yesterday. We re-ran the experiment and found a run where Henge is able to improve performance more. This is the new plot  (Fig~\ref{stepping-utility}).  TODO: We can make the plot interesting by counting the number of reconfigurations required every time new topologies are added. I've removed the description temporarily until I can get the intrusiveness plot}

%\ig{please please max utility.}


Henge stabilizes better when there are more topologies. In the first 2 hours, Fig.~\ref{stepping-utility-a} shows that the average utility of the topologies is below the max, because Henge has less state space to maneuver with fewer topologies. 20 new tenant topologies at the 2 hour mark cause a large drop in  average utility but also open up the state space more--Henge quickly improves system utility to the max value. At the 4 hour and 6 hour marks, more topologies arrive. Henge stabilizes to max utility in both cases. %does not drop as much as it did at the 2 hour mark as more tenants exist on the cluster that have been reconfigured by Henge (the 25 original tenants) and only the new arrivals have to be reconfigured. The same applies when topologies arrive at the 6 hour mark. 

Topologies arriving at the 8 hour mark cause contention. In Fig.~\ref{stepping-utility-a}, the average system utility drops not only due to the performance of the new tenants, but also because the pre-existing tenants are hurt. Henge converges both types of topologies, requiring fewer reconfiguration rounds for the pre-existing topologies (Fig.~\ref{stepping-utility-b}).

%Henge performs fine-grained reconfigurations of both  original and new tenants until they satisfy their SLOs. As shown by Fig.~\ref{stepping-utility-b}, older tenants require fewer rounds of reconfigurations as they had already been reconfigured to meet their SLOs in the past. Thus, Henge is able to adapt topologies to deal with both arrival of new tenants, and poor initial configurations. %to improve low utility caused not only by poor initial configuration but also due to variations caused by arrival of new tenants on a cluster of fixed resources. 
%and 6
 %\ig{avoid verbose explanations.} This is because although Henge reconfigures each topology, one topology's latency does not improve (much like Fig.~\ref{same-step} in Section~\ref{introduction}). When new topologies are added at the 2 hour mark, none of the pre-existing topologies are negatively affected and only the new topologies require reconfiguration, as shown by the red bars in Fig.~\ref{stepping-utility-b}.\fkc{The utility of the previously failing topology also improves. The logs show that although the topology had been physically reconfigured by Henge much earlier, improvements only begin to show at this point.} 

%At the 4 hour mark, we add 20 more topologies: the newly submitted topologies cause variation in the performance of the pre-existing topologies as they take up resources on the cluster, and on average, each pre-existing topology is reconfigured once again to allow it to meet its SLO. As the number of topologies grow on the cluster at the 6 and 8 hour marks, the number of reconfigurations required also grow on average. %At the 6 and 8 hour marks, the additionally added new topologies are reconfigured so they are able to meet their SLOs. 
%\ig{the rest of this para seems fixated on a nit. Talk about the high level points! Remove the rest of this para.} It is noticeable on Fig.~\ref{stepping-utility-a} that reconfiguration begins at an offset to the 6 hour mark. This is because as topologies increase on the cluster, its takes the Nimbus daemon longer to submit new topologies. Henge only performs reconfigurations after all topologies are submitted, to allow the performance of topologies to stabilize. 



%\ig{this para really doesn't say anything interesting or new. Why don't you just say that the system is able to keep up and reach max utility?} 

%\fkc{I had hoped to see more contention for resources in this experiment. Re-running with more tenant topologies (85 instead of 65 to see if we can get better results. More contention means that Henge would rebalance pre-existing topologies more)}




%5,50,95,99 percentile values
% 20.2208920796,25.9907358372,29.3634128485,30.0677037017
% 22.0349340239,30.3363625634,32.2739796203,32.64089089
% 18.1890206599,21.0298438225,24.628927736,27.1511454771
% 0.000756236548566,24.020314323,27.0440825822,30.8578481794
% 34.8752105198,35.0,35.0,35.0








%\ig{All plots must have a horizontal line showing max total utility. Especially important where you are reaching that value, or converging close to it. Don't expect the reader to do math!}





%We evaluate how well Henge is able to handle an increasing number of topologies and cluster sizes, and how it reacts to failures.


\noindent{\bf Increasing Cluster Size:} %We investigate the percentage of SLO achievement Henge can obtain as we scale out the cluster size. 
In Fig.~\ref{scalability} we run 40 topologies on clusters  ranging from 10 to 40 nodes. The machines  have two 2.4 GHz 64-bit 8-core processors, 64 GB RAM, and a 10 Gbps network. 20 topologies are PageLoad with latency SLOs of 80 ms and max utility 35. Among the rest, 8 are diamond topologies, 6 are star topologies and  6 are linear topologies, with juice SLOs of 1.0 and max utility 5.

\begin{figure}[h!]
% 	\vspace{-0.1cm}	
	\includegraphics[width=1.0\columnwidth]{figures/scalability/scalability-combined-10-post-processed.pdf}
	\vspace{-0.7cm}
	\begin{comment}
	\begin{subfigure}{0.5\textwidth}
                \centering
                \includegraphics[width=1\columnwidth]{figures/scalability/scalability-utilities.pdf}%\vspace{-0.1cm}
        \caption{CDF of  topologies according to fraction of their SLO thresholds they are able to reach.}\vspace{-0.1cm}
            \label{scalability-a}
        \end{subfigure}
        \begin{subfigure}{0.5\textwidth}
                \centering
                \includegraphics[width=1\columnwidth]{figures/scalability/scalability-time.pdf}
        \caption{CDF of convergence time for all topologies.}\vspace{-0.1cm}
            \label{scalability-b}
        \end{subfigure}
    \begin{subfigure}{0.5\textwidth}
                \centering
                \includegraphics[width=1.025\columnwidth]{figures/scalability/scalability-intrusiveness.pdf}
                \vspace{-0.7cm}
        \caption{The average number of reconfigurations required per topology to converge, vs. cluster size. }\vspace{-0.5cm} % \ig{these should be bars - only 3 data points. also add median convergence time and fraction of under-SLO topologies. } The CDFs should take care of those
            \label{scalability-c}
        \end{subfigure}
		\end{comment}
		\caption{
		{\bf Scalability w.r.t No. of Machines: }
		\emph{ 40 jobs run on cluster sizes increasing from 10  to 40 nodes. a) CDF of  jobs according to fraction of SLO thresholds reached. b) CDF of convergence time. c) No. of reconfigurations until convergence.}
		}%. all x axes should have same legnths and labels so I can compare. 2. please put more data points than just one (5518, 10497, doesn't tell me anythig about the values aroudn them). 3.The left plot shows the CDF of the amount of time it takes for each topology on a cluster of 30 nodes to achieve its best possible SLO. The right plot correspondingly shows the CDF of the best possible SLO achieved by topologies on the cluster. 
		\label{scalability}

\vspace{-0.3cm}
\end{figure}


%\noindent\textbf
%We measure the impact of increasing cluster size on Henge's performance. \ig{Page Load vs PageLoad - be consistent!}





%\ig{1 give median numbers and 95th percentile and 5th percentiles for each plot. 4. talk about the drop in the rate of topologies not meeting their max utility as the number of machines is increased (you may want to add that line to the fig 26 plot). 5. talk about the trend in the median convergence time as a function of cluster size (also add this to fig 26).}

%\ig{please spend time on explaining the plot and describing it in detail, especially tangible points of the plot. the description seems hurriedly written at this point.}

% In all settings at least 40\% of topologies are able to meet their SLO threshold.

%At the 95th percentile, topologies on even the 10 node cluster are able to achieve their SLO, .

%\ig{that last sentence needs to be described more clearly and in layman terms.}

%\ig{every para needs to have a point it is tryin to make. make it quickly and crisply, then move on.}

%At the 5\% percentile, topologies provide 56.4\%,  75.4\% and 94.5\% SLO satisfaction on cluster sizes of 20, 30, and 40 nodes respectively. With 20-40 nodes, median topologies are able to fully satisfy their SLO. However, at the median and 95\% percentile, topologies in all settings are able to meet their SLOs. On clusters of larger sizes, the CPUs are slower to saturate, allowing room for further improvement.


\begin{comment}
utility: (5\%, 50\%, 95\%)

utility:
10: 0.00291784, 0.04604453, 1
20: 0.56438447, 1, 1
30: 0.73958849, 1, 1
40: 0.94455272, 1, 1

time:
10: 0, 537.177, 11895.183
20: 0, 2807.55, 5866.216
30: 0, 1761.399, 4200.567
40: 0, 2225.875, 10573.931
\end{comment}

% \ig{next sentence is very complex and needs rewriting.}

From Fig.~\ref{scalability}a, Henge is able to provide SLO satisfaction for 40\% of the tenants even in an overloaded cluster of 10 nodes. As expected, in large clusters Henge has more room to maneuver and meets more SLOs. This is because CPUs saturate slower in larger clusters. In an overloaded cluster of 10 nodes, topologies at the 5th percentile are able to achieve only 0.3\% of their max utility. On the other hand, in clusters with 20, 30, and 40 machines, 5th percentile SLO satisfactions are higher: 56.4\%, 74.0\% and 94.5\% respectively. 

%topologies above the 60th percentile are able to achieve their SLOs on all cluster sizes. This means that even on an overloaded cluster of 10 nodes, Henge is able to provide SLO satisfaction for 40\% of the tenants.

%In all settings, all topologies above the 60th percentile achieve their SLOs; thus even in overloaded situations Henge improves the SLO satisfaction of at least 40\% of the existing tenants.


Fig.~\ref{scalability}b shows the time taken for topologies to converge to their highest utility.  Interestingly, while the 10 node cluster has a longer tail than 20 or 30 nodes, it converges faster at the median (537.2 seconds). %, vs. for 2225.9 seconds for 40 nodes. % it is , which is 4.1$\times$ greater. 
Topologies at the tail of both the 10 and 40 node clusters take a longer time to converge. This is because in the 10 node cluster, greater reconfiguration is required per topology as there is more resource contention (see Fig.~\ref{scalability}c). At 40 nodes, collecting cluster information from  Nimbus daemons leads to a bottleneck. This can be alleviated by decentralized data gathering (beyond our scope). %This is not a fundamental limitation and could be alleviate by decentralized data gathering (Statistics Module). 

%. This is because Henge runs as part of the centralized Nimbus daemon and gathers low-level metrics from the entire cluster to make global decisions: the larger the cluster, the greater the communication cost to the centralized scheduler. The scalability of Henge could be improved by decentralizing the Statistics module, to trade off metric staleness and reconfiguration accuracy for better scalability. (This is beyond our scope.) %\ig{this last part of this para is going off on a tangent. this is the kind of thing that bores reviewers (and hurts your paper). stick to the point!} \fkc{I need this to explain the results.}
%  We found from our deep dive for the 40 node cluster that the long tail for convergence is because of a reduction step that reduced CPU load on the cluster nodes, but caused some SLO misses, requiring further reconfiguration. % topologies to miss their SLO.  

Fig.~\ref{scalability}c shows that the number of reconfigurations needed to converge is at most 2 $\times$ higher when resources are limited and does not otherwise vary with cluster size. Overall, Henge's performance generally improves with cluster size, and overheads are scale-independent. % showing Henge's scalability. 



\subsubsection{Fault Tolerance}


Henge reacts gracefully to failures. In Fig.~\ref{fault-tolerance}, we run 9 topologies each with 70 ms SLO and 35 max utility. We introduce a failure at the worst possible time: in the midst of Henge's reconfiguration operations, at 1020 s. This severs communication between Henge and all the worker nodes; and Henge's Statistics module  is unable to obtain fresh information about jobs. We observe that Henge reacts conservatively by avoiding reconfiguration in the absence of data.  %as it cannot determine whether  worker nodes are dead and cannot receive updates about improving performance. 
At 1380 s, when communication is restored, Henge collects performance data for the next 5 minutes (until 1680 s) and then proceeds with reconfigurations as usual, meeting all SLOs. 

\begin{figure}[h!]
 	\vspace{-0.1cm}	
	\begin{center}%exp158
\includegraphics[width=1.0\columnwidth]{figures/failure-utility/failure-utility.pdf}\vspace{-0.3cm}
%exp158 ()
\caption{{\bf Fault-tolerance:} \it Failure occurs at t=1020s, and recovers at t=1380 s. Henge makes no wrong decisions due to the failure, and immediately  converges to the max system utility after recovery. }
		\vspace{-0.5cm}
		\label{fault-tolerance}
	\end{center}

\end{figure}


\subsection{Memory Utilization}
\label{sec:memory-utilization}


Fig.~\ref{memory-utilization} shows a Henge cluster with 8 memory-intensive topologies. Each topology has a max utility value of 50 and a latency SLO of a 100 ms. These topologies have join operations, and tuples are retained for 30 s, creating memory pressure at some cluster nodes. As the figure shows, Henge reconfigures memory-bound topologies quickly to reach total max utility of 400 by 2444s, and keeps  average memory usage below 36\%. Critically, the memory utilization (blue dotted line) plateaus in the converged state, showing that Henge is able to handle memory-bound topologies gracefully.


\begin{figure}[ht]
% 	\vspace{-0.2cm}	
	\begin{center}%results/exp43
\includegraphics[width=1.0\columnwidth]{figures/memory/memory.pdf}
\vspace{-0.75cm}
\caption{{\bf Memory Utilization:} \emph{ 8 jobs with joins and 30 s tuple retention.}}   
		\vspace{-0.5cm}
		\label{memory-utilization}
	\end{center}
\end{figure}

%Effectively, Henge tries to spread work equally across machines and reduce congestion on individual operators. We evaluate Henge to ensure that it can also handle a memory intensive workload. We run a simple topology that has two spouts, which emit {\tt [id, gender]} and {\tt [id, age]} respectively. A downward bolt receives these tuples and performs a join based on id. The memory consumption of the bolt can be large as tuples are retained in memory for upto 30 seconds until their pair arrives. We run 8 of these topologies, each with a latency SLO of 100 ms on a 20 node cluster. We observe that while Henge performs reconfiguration, average memory utilization across the cluster drops and converges to a low percentage once all topologies meet their SLO.
























\begin{comment}
\subsection{Henge Policy and Scheduling (DEPRECATED)}

We experimentally show how Henge's scheduling policy meets several requirements: a) Reacting to SLO misses; b) Dealing with workload variations; c) Dealing with different kinds of SLOs; d) Scaling with number of topologies; and e) Helping with consolidation of cluster resources.


\subsubsection{Meeting SLOs}

\noindent {\bf One Missing SLO:} We start with the simplest case where a single topology misses its SLO on a cluster. Fig.~\ref{microbenchmark-slo} shows the juice and utility values of three juice-sensitive topologies each with juice SLO = 1.0 and max  utility = 5. T1 is a linear topology, T2 is diamond topology and T3 is a star topology. T2 is unable to achieve its SLO by 900 s. Immediately after the waiting period is over (900 s), Henge performs resource reallocation and in three successive reconfigurations, all topologies meet its SLO by 1081 s. 

\noindent {\bf Equal Utilities, Multiple Misses: }  Fig.~\ref{equal} is a case where all five PageLoad topologies (latency SLO 80 ms, max utility 35 each) are initially unable to meet their SLO.  Henge quickly performs one reconfiguration for each topology, within a short interval from 900 s to 1109 s, allowing all topologies to meet their respective SLOs. 


\noindent {\bf Unequal Utilities, Mix of Latency and Juice SLOs:} 

We further complicate the workload where three topologies have latency SLOs (T1-T3, 80 ms SLOs with max utility 35) and the other two have juice SLOs (T4-T5, 1.0 SLOs with max utility 5). Fig.~\ref{unequal} shows the timeline.




Initially, total utility converges at a value of 10.04. The main contributors to this sum are T4 and T5, which are very close to their SLOs.  When Henge does reconfiguration  (indicated by solid black lines), it chooses topologies in the following order: T1, T2, T3, and T4  by 1132 s.  After T1, T2 and T3 are reconfigured, total utility reaches 119.78, very close to the maximum achievable value of 120. Henge is minimally intrusive: it reconfigured each topology exact once during this run. 


\noindent{\bf SLO Achievement with Limited Resources:} 

Fig~\ref{reversion-reduction} presents system utility of an overloaded cluster. We investigate the improvement in performance Henge can provide. There are 4 diamond, 3 linear and 3 star topologies running, each with utility values of 5 and juice SLOs of 1.0. Henge reconfigures the topologies until they stop showing further improvement, and the system initially converges to a total utility of 47. At 35900 s, a drop in total utility is correlated with very high CPU load. After a period of stability, Henge recognises drops in utility only if current utility is less than 5\% best-seen utility. After total utility drops below this threshold, Henge performs reduction, to reduce CPU load. 


Henge finds only two topologies (T8 and T10) that meet their SLO, and subjects them to reduction at 35961 s. When T8 is reduced the system utility improves marginally (solid line) but T8's own utility drops, and thus Henge subsequently reconfigures it. However, this further drops T8's utility, indicating a wrong path in the search space. Thus Henge merely reverts back to the reduced configuration which provided total maximum utility of 44.72. As compared to the initially low utility, this configuration increases total utility by 10\% . 

\paragraph{Preventing Resource Hogging}
Henge does not allow a topology to unfairly hog resources. This may  especially occur when a topology has an SLO that is impossibly stringent for current resources. 


Fig~\ref{fairness} shows 5 PageLoad topologies running on a cluster. (T1-T3)  have stringent SLOs of 5ms and max utilities of 20 each. T4-T5 have juice SLOs of 1.0 and max utilities of 5.


Solid black lines on the plot mark topology reconfigurations. The broken lines indicate instances where T1-T3 don't meet their SLOs but they are not  given resources; this is because their last reconfiguration improved utility by less than 5\%. 
The first round of reconfiguration occurs at 900 s. T1-T3 are reconfigured multiple times by 1306 s  and T4-T5 rebalance once by 1516 s. After these rebalances, T1-T3 are blacklisted for an hour from further reconfigurations as they do not show sufficient improvement. To allow topologies to receive as much resources as they can, Henge reconfigures T1-T3 after another hour (starting from 4787 s) as resources are still available. Nevertheless, significant improvement is not seen and so, T1-T3 are not reconfigured again. In other words, for potentially hoggy topologies, Henge attempts to reconfigure them far rarely than otherwise well-behaved topologies.



\subsubsection{Workload Variations}

\vspace{-0.5em}\paragraph{Spike in Rates:} Fig.~\ref{spike} shows the input rate of topologies spiking suddenly at time t=4000s, with traffic increasing 3 $\times$.



 Five latency-sensitive topologies are run, each with SLO of 80ms and maximal utility values of 35.  When the spike occurs at 4000 s, operators in the  topologies start to become congested, dropping system utility from 175 to 172.8. At this moment, Henge performs resource reconfiguration. By 5048 s, Henge is able to bring the utility back up to 173.9. By t=5743s, total utility is back up to maximum utility.  


Henge incurs very few reconfigurations for individual topoplogies. The maximum number of reconfigurations required were 3, for T1, and the minimum was 1, for T2, T4 and T5.  This reduces intrusion by Henge. At t=8000s, we allow the spike to elapse and input rate to return to original values; this results in no further reconfigurations.



\paragraph{Diurnal Rates}
 A stream processing system will face a diurnal variation of input rate, especially for e-commerce websites~\cite{decandia2007dynamo} and social media~\cite{naaman2012study}.  
 To model this, we generate a  workload based on the distribution of the SDSC-HTTP traces~\cite{web-trace}. We change the workload of the PageLoad topology to reflect this distribution. Results are shown in Fig.~\ref{diurnal}. Each hour of the workload maps to a 10-minute interval in the experiment. This workload increases from 7th hour of the day, reaches its peak at 14th hour (8400 s) and starts to decrease. At 7th hour (4200 s) of the workload, the pageload topology violates its SLO, and Henge accordingly performs reconfiguration. During the workload increase Henge performs 9 consecutive rebalances in order to adapt to the load. By the time the workload reaches its peak at 14th hour, the system has adapted to the workload change and no further rebalances need to be triggered.
 


\vspace{-0.2cm}
\subsubsection{Types of SLOs} 
In addition to latency and juice SLOs, Henge can also support the following kinds of performance SLOs.

\paragraph{Tail Latencies}

While Henge adopts average latencies for SLOs, it can be extended to satisfy tail latency SLOs. To show that Henge improves tail latencies, we point the reader to 
Fig.\ref{equal} which also shows the 99th percentile tail latency values. Every time a reconfiguration occurs, tail latencies improve.


\paragraph{Hybrid SLOs} Recently, authors from Facebook say~\cite{facebook-slos} that as they persist all data to disk, they have to tolerate higher latency (although with an upper bound) while having very high throughput. In such a scenario, topologies can have a ``hybrid'' SLO that consists of both a maximum tolerable latency and a minimum processing rate as compared to the input rate.

We evaluate an example (Fig.~\ref{hybrid}) where 4 hybrid topologies are run on a cluster. We consider the case of T2 which has a juice SLO of 1.0 and a latency SLO of 50 ms. A hybrid SLO needs both of its requirements satisfied. It has separate utility functions for juice and for latency, and the job's utility is the average value of these two utilities. 

Henge is greedy and tries to meet the closer SLO (juice or latency) for a given topology. In this instance, the easier SLO is the juice SLO, which is satisfied first at 988 s.  As Henge tries to un-congest operators to improve juice, latency decreases but does not sufficiently to meet the SLO. A second reconfiguration is needed at  1120 s to meet the latency SLO. In all, Henge requires only two reconfigurations to meet this hybrid SLO.



\subsubsection{Scalability}
\begin{figure}[h!]
	\vspace{-0.4cm}
	\begin{center}
		\includegraphics[width=1\columnwidth]{figures/scalability-terms.pdf}
		\vspace{-0.4cm}\caption{As the number of topologies on a cluster increase, the waiting time for each to be reconfigured increases linearly. However, once a topology is chosen, it is completely reconfigured in 2 or fewer rounds.}
		\label{scalability}
	\end{center}
\vspace{-0.5cm}
\end{figure}




When Henge starts reconfiguring a set of topologies, it may: a) take a while before all topologies reach their SLO as it goes through topologies iteratively (i.e., system convergence time) and b) once it reaches a particular topology $T$, it may take a few rounds to bring $T$ up to its SLO (total topology reconfiguration time). Fig.~\ref{scalability} shows these two metrics respectively. From the first plot we notice that system convergence time grows linearly (all topologies are PageLoad); this is expected as Henge is conservative in not picking too many topologies to reconfigure simultaneously. However, once a topology is touched, it is configured very quickly, and in a time that is indepedendent of the number of jobs. Further, no topology took longer than 2 rounds to converge. This shows that Henge's primary decision making in giving or taking away resources, is highly effective and scalable. 




\subsubsection{Resource Consolidation} %\ig{Indy placeholder: not read} 
\begin{figure}[h!]
	%\begin{wrapfigure}{r}{0.5\textwidth}
	\vspace{-0.4cm}
	\begin{center}
		\includegraphics[width=1\columnwidth]{figures/optimality/optimality.pdf}\hfill
	\end{center}
	\vspace{-0.5cm}
	\caption{ With or without sufficient resources, Henge allows topologies to show improved utility than they would without it.} 
	\label{optimality}
	\vspace{-0.3cm}
	%\end{wrapfigure}
\end{figure} 


	We next measure how effectively Henge consolidates resources. We use 5 PageLoad topologies with maximal utilities of 20, two with latency SLOs of 80ms and the remaining with SLOs of 20ms. Fig.~\ref{optimality} shoss that when the cluster size is small, there are insufficient resources to reach the maximum utility. Henge only needs 3 machines to reach the maximum system utility. If each of the 5 topologies were given static clusters (no multi-tenancy), a minimum of 5 machines would have been required to achieve maximum utility. Thus in this case, Henge reduces total capital expenses by 2/5 - 40\%.
\end{comment}

\begin{comment}
\begin{figure}[h!]
	\begin{center}
\includegraphics[width=0.8\columnwidth]{figures/placeholders/slo-stringency.jpeg}
\caption{Stringent SLOs require more resources to be met.}
		\label{slo-stringency}
	\end{center}
\vspace{-0.2cm}
\end{figure}


\begin{figure}[h!]
	\vspace{-0.5cm}	
	\begin{center}
\includegraphics[width=0.8\columnwidth]{figures/placeholders/intrusiveness-topology-number.jpg}
\caption{As the number of topologies increase on the cluster, more reconfiguration is required to improve the performance of each topology and manage the CPU bottleneck.}
		\label{topology-intrusive}
	\end{center}
\vspace{-0.2cm}
\end{figure}


\vspace{1cm}
\begin{figure}[h!]
	\vspace{-0.5cm}	
	\begin{center}
\includegraphics[width=0.4\columnwidth]{figures/discussion-figures/scalability/35-time.pdf} 
\includegraphics[width=0.4\columnwidth]{figures/discussion-figures/scalability/35-util.pdf} 
\caption{The left plot shows the CDF of the amount of time it takes for each topology on a cluster of 35 nodes to achieve its best possible SLO. The right plot correspondingly shows the CDF of the best possible SLO achieved by topologies on the cluster. }
		\label{discussion:35}
	\end{center}
\vspace{-0.2cm}
\end{figure}

\vspace{1cm}
\begin{figure}[h!]
	\vspace{-0.5cm}	
	\begin{center}
\includegraphics[width=0.4\columnwidth]{figures/discussion-figures/scalability/40-time.pdf} 
\includegraphics[width=0.4\columnwidth]{figures/discussion-figures/scalability/40-util.pdf} 
\caption{ The left plot shows the CDF of the amount of time it takes for each topology on a cluster of 40 nodes to achieve its best possible SLO. The right plot correspondingly shows the CDF of the best possible SLO achieved by topologies on the cluster.}
		\label{discussion:40}
	\end{center}
\vspace{-0.2cm}
\end{figure}

\subsubsection{Intrusiveness on larger clusters}
\vspace{1cm}
\begin{figure}[h!]
	\vspace{-0.5cm}	
	\begin{center}
\includegraphics[width=1.0\columnwidth]{figures/discussion-figures/scalability/intrusiveness.pdf} 

\caption{}
		\label{discussion:intrusiveness}
	\end{center}
\vspace{-0.2cm}
\end{figure}

\vspace{1cm}
\begin{figure}[h!]
	\vspace{-0.5cm}	
	\begin{center}
\includegraphics[width=0.8\columnwidth]{figures/placeholders/intrusiveness-cluster.jpg}
\caption{As the cluster size increases, topologies do not face a resource bottleneck and require fewer resources.}
		\label{cluster-intrusive}
	\end{center}
\vspace{-0.2cm}
\end{figure}
\end{comment}


% old stateful stuff
% \ig{Writing could be compressed.} We present an example where a topology with at-most once semantics checkpoints regularly in Redis. 
% Fig.~\ref{stateful} shows a CDF of the fraction of time stateful topologies provide a given utility. Two topologies are run in the experiment, each with a utility of 35 and a latency SLO of 500ms. These topologies are performing a stateful word count. The input rate of T1 is higher and mirrors the ``Egypt" input rate, whereas the input rate of T2 mirrors the  input rate from the ``London" workload, described in Table~\ref{table:yahoo-job-dist}.  The count of words is updated in a Redis installation and the final updated count is printed by the sink bolt. The wait-time for insertion and reading from Redis is an overhead for the topologies, which is why the latency SLO is set to 500ms. At the $5^{th}$ percentile, both topologies are unable to provide full utility -- T1 has a utility of 0.176 and T2 has a utility of 0.319. By the $25^{th}$ percentile, T1 has risen to 1.811  and T2 provides its full utility of 35. By the $40^{th}$ percentile, T1 increases to 8.589 and by the $50^{th}$, it too provides full utility.

% \begin{figure}[h!]
% 	%\vspace{-0.6cm}	%stateful exp  %exp3 -- d710
%             \centering
%         \includegraphics[width=1\columnwidth]{2017-09-02/figures/stateful/util-cdf.pdf}\vspace{-0.3cm}
% \caption{{\bf Stateful Topologies in Henge: } \it CDF of the fraction of total time stateful tenant topologies provide a given SLO satisfaction. Max utility for each topology is 35.} 
%     \label{stateful}
%  \vspace{-0.3cm}
% \end{figure}

==> henge-arxiv 2/text/11c-henge-policy-eval-figs.tex <==
\begin{figure*}
	\centering
	\begin{minipage}{1\columnwidth}
		\centering
		\includegraphics[width=1\columnwidth]{figures/simple-convergence/exp72/figure14.pdf} % \
		\caption{Right top: Topologies are chosen for reconfiguration based on which has worst performance. Right bottom: The improvement in total utility due to reconfiguration. Left: $99^{th}$ percentile latency improves due to reconfigurations. \fkc{Don't use moving average for tail latency}	}	\label{equal}
	\end{minipage}\hfill
	\begin{minipage}{1\columnwidth}
		\centering
		\includegraphics[width=1\columnwidth]{figures/simple-convergence/exp109/figure15.pdf} % second figure itself
		\caption{Topologies are chosen for reconfiguration, first in order of priority, and second in order of poor performance. Therefore, the T1-T3 are chosen first (utility=35), and T4 (utility=5) is chosen last. Right bottom: reconfiguring T1-T3 provides most increase in overall utility. \fkc{Make points bigger}
		}
	
				\label{unequal}
	\end{minipage}
\end{figure*}

\begin{figure}[t]
	\vspace{-0.7cm}
	\centering
	\includegraphics[width=0.8\columnwidth]{figures/reversion.pdf}
			\vspace{-0.2cm}
		% This is exp 134
	\caption{A cluster of 10 topologies (utility of each topology=5) converges after reversion}
	\label{reversion-reduction}
\end{figure}

\begin{figure}[h!]
	\vspace{-0.5cm}	
	\begin{center}
				\includegraphics[width=1.0\columnwidth]{figures/hybrid/hybrid.pdf}
			\caption{Hybrid SLOs: the first and second reconfiguration help meet the juice and latency SLO respectively }
			
		\label{hybrid}
	\end{center}
\vspace{-0.2cm}
\end{figure}



\begin{figure}[t]
	\vspace{-0.3cm}	
		\begin{center}
			\includegraphics[width=1.0\columnwidth]{figures/fairness/all.pdf}
    \caption{Topologies are no longer reconfigured (during time indicated in dotted green) as they do not show more than 5\% improvement in last reconfiguration}
	\label{fairness}
			\end{center}
		\vspace{-0.6cm}	
\end{figure}
	


\begin{figure*}
	\centering
	\begin{minipage}{1\columnwidth}
				\vspace{-0.6cm}
		\centering
		\includegraphics[width=1\columnwidth]{figures/simple-convergence/exp95/figure19.pdf} % first figure itself

		\vspace{-0.3cm}
		\caption{Reconfiguration allows a topology to adjust to a spike in input rate}
		\label{spike}
		\vspace{-0.5cm}
	\end{minipage}\hfill
	\begin{minipage}{1\columnwidth}
				\vspace{-0.5cm}
		\centering
		\includegraphics[width=1\columnwidth]{figures/diurnal/diurnal_2.pdf} % second figure itself
		\caption{Diurnals are a common pattern in internet traffic. Henge reconfigures a topology so it is able to meet its SLO of 60 ms during peak loads.}
		\label{diurnal}
				\vspace{-0.1cm}
	\end{minipage}

\end{figure*}


==> henge-arxiv 2/text/12-related-work.tex <==
\vspace{-0.3cm}
\section{Related Work}
\label{related-work}

%\ig{Indy placeholder: not read}


\noindent {\bf Elastic Stream Processing Systems:}
Traditional query-based stream processing systems such as Aurora~\cite{aurora} and Borealis~\cite{borealis} provide load-balancing~\cite{load-in-borealis} but not first-class multi-tenant elasticity. 
Modern general-purpose stream processing systems~\cite{flink,flume,samza,storm_web,s4,akidau2013millwheel,heron,naiad} do not natively handle adaptive elasticity. Ongoing work~\cite{spark-elasticity}  on Spark Streaming~\cite{spark_streaming} allows scaling but does not apply to resource-limited multi-tenant clusters.~\cite{seep,timestream} scale out stateful operators and  checkpoint, but do not scale in or support multi-tenancy. %TimeStream~\cite{timestream} describes resilient substitution as a single method for fault recovery and resource reconfiguration without addressing the multi-tenancy problem. %~\cite{seep,seep-poster} describe a single approach for scaling out stateful operators and recovering from failures based on check-pointing but do not discuss scale-in or resource distribution in the presence of multiple tenants. Similarly, TimeStream~\cite{timestream} describes resilient substitution as a single method for fault recovery and resource reconfiguration without addressing multi-tenancy.

%{\bf Elastic Stream Processing Systems:} Aurora~\cite{aurora} and Borealis~\cite{borealis} are seminal stream processing systems.  Borealis does load balancing in a static environment~\cite{load-in-borealis}, but does not handle elasticity.  Distributed stream processing systems based on the continuous operator model~\cite{flink,flume,samza,storm_web,s4,akidau2013millwheel,heron,naiad} process records from queues and provide varying levels of fault-tolerance, but do not provide adaptive elasticity. Spark Streaming~\cite{spark_streaming} processes data streams in micro-batches. Ongoing~\cite{spark-elasticity} work on Spark Streaming~\cite{spark_streaming} allows scaling but does not apply to resource-limited multi-tenant clusters. ~\cite{seep,seep-poster,timestream} describe scale out of stateful operators,  check-pointing, and reconfiguration but not scale-in or multi-tenancy. %TimeStream~\cite{timestream} describes resilient substitution as a single method for fault recovery and resource reconfiguration without addressing the multi-tenancy problem.

Resource-aware elasticity in stream processing~\cite{balkesen2013adaptive,cervino2012adaptive,fu2015drs,kalyvianaki2012overload,kleiminger2011balancing,satzger2011esc,peng2015r}   assumes infinite resources that the tenant can scale out to. %focus on optimizing individual tenants' performance individually while assuming infinite extra resources abound.
~\cite{aniello2013adaptive,elastic-scaling-system-S,jain2006design,li2015supporting,stormy,schneider2009elastic,wu2007challenges} propose  resource provisioning but not multi-tenancy. Some works have focused on balancing load~\cite{twochoices,morethantwochoices}, optimal operator placement~\cite{SQPR,network-aware-placement,heinze2014latency} and scaling out strategies~\cite{heinze2014auto,heinze2015online} in stream processing systems. These approaches can be used in complement with Henge in various ways. \cite{heinze2014latency,heinze2014auto,heinze2015online} look at single-job elasticity, but not multi-tenancy.% These  approaches are orthogonal to Henge and can complement it.

%SQPR~\cite{SQPR}  models query admission, allocation, and operator reuse, as an  optimization problem with an approximate solution. 






Themis'~\cite{kalyvianaki2016themis} SIC %fairly sheds tuples in an overloaded, federated stream processing system to achieve balanced query performance. While its proposed SIC 
metric is similar to juice, but Themis uses SIC to drop tuples. Henge does not drop tuples. 
%but the two systems have different goals. Themis measures the weight of each tuple to find those that can be dropped to reduce load, while Henge uses juice to support SLOs.
Dhalion~\cite{floratou2017self} supports throughput SLOs for Heron, but it is unclear how this generalizes to varying input rates. It uses topology backpressure as a trigger for scaling out topologies, but because backpressure takes a while to propagate (e.g., after a spike), this approach is less responsive than using CPU load. %It uses topology backpressure to trigger scale out, but backpressure responds sluggishly to spikes than does CPU load. %

%Dhalion~\cite{floratou2017self} describes a system that provides the capabilities of self-regulation to stream processing systems, namely Heron. It only supports throughput SLOs and uses triggers such as backpressure to detect whether a single topology is failing and then carries out dynamic resource provisioning to resolve the issue. However, backpressure is a very coarse-grained measure of SLO satisfaction -- by the time backpressure is triggered, a latency SLO  in place by the user may already be violated. In addition, backpressure completely stops tuples flowing in the topology, meaning that resources are consumed for a topology even though it is doing no work. Henge simply uses SLO violations as a trigger for corrective measures and is able to satisfy both latency and throughput SLOs in a multi-tenant environment.

\noindent {\bf Multi-tenant Resource Management Systems:} Resource schedulers like  YARN~\cite{yarn} and Mesos~\cite{mesos} can be run under stream processing systems, and manually tuned~\cite{cloudera:yarn-tune}.
%However, they do not provide specific insight into the performance of stream processing jobs. 
Since the job internals are not exposed to the scheduler (jobs  run on containers) it is impossible to make fine-grained decisions for stream processing jobs in an automated fashion. %, but there is no work on adaptivity  in these resource managers. 

\noindent {\bf Cluster Scheduling: } Some systems propose scheduling solutions to address resource fairness and SLO achievement~\cite{delimitrou2013paragon, quasar, ghodsi2011dominant, mace2015retro, rameshan2016hubbub, shue2012performance}. %Hubbub~\cite{rameshan2016hubbub} considers how interference from other tenant VMs in a cluster can effect performance and performs scaling accordingly so that SLOs are met. There is little discussion of how SLOs are defined or set. 
VM-based scaling approaches~\cite{vm-based} do not map directly and efficiently to expressive frameworks like stream processing systems. %, which is why a system like Henge is needed.   %As opposed to these approaches and other (virtual machine based approach such as~\cite{vm-based}), Henge leverages the knowledge of Storm architecture to perform dynamic resource reconfiguration to maximize performance.
%Retro~\cite{mace2015retro} manages resources for distributed systems but is not elastic. 
Among multi-tenant stream processing systems, Chronostream~\cite{wu2015chronostream} achieves elasticity through  migration across nodes. It does not support SLOs.  %Elasticity ideas from batch processing  (Amoeba~\cite{elastic-multi-tenant-compute-cluster}) are hard to apply to stream processing. 
%Cloudscale~\cite{shen2011cloudscale} minimizes energy/power used (assuming infinite resources) while meeting SLOs. 
%Initial operator placement strategies like~\cite{heinze2014latency,heinze2014auto,heinze2015online,lohrmann2015elastic} can be combined with Henge. %are orthogonal to Henge and could be integrated with it.



%\noindent {\bf Storage/Transaction Processing Systems:} %E-store~\cite{e-store}  re-distributes hot and cold data chunks across nodes in a cluster. Cake~\cite{wang2012cake} supports latency and throughput requirements in multi-tenant storage settings. %handles the challenge of scheduling data store queries with both latency and throughput requirements in a multi-tenant environment, using a two-level scheduling technique. These techniques generally involve splitting the location of hot data and cannot be applied to stream processing systems.

\noindent {\bf  SLAs/SLOs in Other Areas:} %Work on distributed systems storage has looked at satisfying latency and consistency SLOs. For example, 
SLAs/SLOs have been explored in other areas. %, especially distributed storage. 
Pileus~\cite{terry2013consistency} is a geo-distributed storage system that supports multi-level SLA requirements dealing with latency and consistency. %During favorable conditions, the system can deliver responses with ideal consistency and latency. When conditions deteriorate, it refers to the user's SLA specification to decide whether to prefer consistency or low latency when fetching results.
Tuba~\cite{ardekani2014self} builds on Pileus and performs reconfiguration to adapt to changing workloads. 
SPANStore~\cite{wu2013spanstore} is a geo-replicated storage service that automates trading off cost vs. latency, while being consistent and fault-tolerant. 
%SPANStore~\cite{wu2013spanstore} is a geo-replicated storage service that spans multiple cloud services and automates the process of trading off cost and latency, while being consistent and fault-tolerant. 
E-store~\cite{e-store}  re-distributes hot and cold data chunks across nodes in a cluster if load exceeds a threshold. Cake~\cite{wang2012cake} supports latency and throughput SLOs in multi-tenant storage settings.


%To the best of our knowledge, Henge is the first work that combines SLOs and elastic resource management for stream processing systems in a multi-tenant environment.


\begin{comment}

\section{Related Work}
\label{related-work}

{\bf Elastic Stream Processing Systems:} Aurora~\cite{aurora} and Borealis~\cite{borealis} are seminal stream processing systems.  Borealis does load balancing in a static environment~\cite{load-in-borealis}, but does not handle elasticity.  Distributed stream processing systems based on the continuous operator model~\cite{flink,flume,samza,storm_web,s4,akidau2013millwheel,heron,naiad} process records from queues and provide varying levels of fault-tolerance, but do not provide adaptive elasticity. Spark Streaming~\cite{spark_streaming} processes data streams in micro-batches. Ongoing~\cite{spark-elasticity} work on Spark Streaming~\cite{spark_streaming} allows scaling but does not apply to resource-limited multi-tenant clusters. ~\cite{seep,timestream} describe scale out of stateful operators,  check-pointing, and reconfiguration but not scale-in or multi-tenancy. %TimeStream~\cite{timestream} describes resilient substitution as a single method for fault recovery and resource reconfiguration without addressing the multi-tenancy problem.

Many systems have focused on resource-aware elasticity in stream processing systems~\cite{balkesen2013adaptive,cervino2012adaptive,fu2015drs,kalyvianaki2012overload,kleiminger2011balancing,satzger2011esc}. Stormy~\cite{stormy} allows scaling by partitioning queries across nodes, however, it is subject to inconsistent decisions as any node in the cluster can make a scaling decision--in comparison, Henge has a consistent global view. 

Single-tenant performance optimizations assuming infinite extra resources abound for stream processing. \cite{aniello2013adaptive} places operators to minimize communication and \cite{elastic-scaling-system-S,schneider2009elastic} tune parallelism of operators in System S~\cite{jain2006design,wu2007challenges} on multi-cores. \cite{li2015supporting} addresses resource provisioning for stream processing applications with latency constraints without addressing multi-tenancy.

Themis~\cite{kalyvianaki2016themis} describes an algorithm that fairly sheds tuples in an overloaded, federated stream processing system to achieve balanced performance across queries. Although its proposed SIC metric is similar to the juice metric in Henge, the goals of the two systems are dissimilar. Henge requires a measure of overall job performance in terms of throughput to maximise the number of tuples processed per unit time and meet SLOs. Conversely, Themis measures the weight of each tuple to discover those that can be dropped to reduce load. 

Some works have focused on balancing load and optimal operator placement in stream processing systems. Nasir et al., apply the power of two choices to a distributed stream processing system by locally estimating load of parallel instances of operators and splitting keys between them~\cite{twochoices}. Since this approach involves replicating state for stateful operators, they propose~\cite{morethantwochoices}, where they deduce the minimum number of parallel instances of operators required on which state must be replicated, based on the skew of the input distribution.~\cite{network-aware-placement} prioritizes efficient use of the network and describes a stream-based overlay network that manages operator placement for stream processing systems. SQPR~\cite{SQPR} describes a static scheduler that models query admission, allocation, and operator reuse as a single complex optimization problem and then solves an approximate version. These approaches are orthogonal to Henge and can be used to complement it.
\vspace{-1.5em}\paragraph{Resource Management in Storage/Transaction Processing Systems:} E-store~\cite{e-store} is an elastic partitioning framework for distributed transaction processing systems which intelligently re-distributes hot and cold data chunks across nodes in a cluster when load exceeds a certain threshold. Cake~\cite{wang2012cake} handles the challenge of scheduling data store queries with both latency and throughput requirements in a multi-tenant environment, using a two-level scheduling technique. These techniques generally involve splitting the location of hot data and cannot be applied to stream processing systems.
\vspace{-1.5em}\paragraph{Multi-tenant Resource Management Systems:} Apache Yarn~\cite{yarn} and Mesos~\cite{mesos} are two recent resource managers that are used for multi-tenant clusters and can run stream processing systems. However, they do not provide any more insight into the performance of stream processing job any more than standalone systems. Further, it is more difficult to make fine-grained optimizations as the internals of jobs aren't exposed to the schedulers (jobs are usually run in containers on host machines). Various articles describe how to manually tune Yarn to provide the best performance e.g.,~\cite{cloudera:yarn-tune}, however, very little work on adaptive scheduling is found for these resource managers.

Omega~\cite{Schwarzkopf:2013:OFS:2465351.2465386} is a scheduler that has targeted SLOs while providing Dominant Resource Fairness~\cite{ghodsi2011dominant}. Pisces~\cite{performance-isolation-fairness} has focused on providing fairness in key-values stores. Paragon~\cite{delimitrou2013paragon} is intended for multi-tenant distributed systems but assumes infinite resources. Quasar~\cite{quasar} is a cluster management system that uses classification methods to performs coordinated resource allocation and assignment. It currently supports distributed analytics frameworks, web-serving applications, NoSQL datastores, and single-node batch workloads.
Hubbub~\cite{rameshan2016hubbub} considers how interference from other tenant VMs in a cluster can effect performance and performs scaling accordingly so that SLOs are met. There is little discussion of how SLOs are defined or set. As opposed to these approaches and others (\cite{vm-based} based on hardware virtualization), Henge leverages the knowledge of Storm architecture to perform dynamic resource reconfiguration to maximize performance.

Retro~\cite{mace2015retro} manages resources for distributed systems but is not elastic. Among multi-tenant stream processing systems, Chronostream~\cite{wu2015chronostream} achieves elasticity through workload migration across nodes. It does not support SLOs.  %Elasticity ideas from batch processing  (Amoeba~\cite{elastic-multi-tenant-compute-cluster}) are hard to apply to stream processing. 
Cloudscale~\cite{shen2011cloudscale} minimizes energy/power used (assuming infinite resources) while meeting SLOs. This, and other works~\cite{heinze2014latency,heinze2014auto,heinze2015online,lohrmann2015elastic} which reduce latency in stream processing by considering operator placement, are orthogonal to Henge and could be integrated with it.% our system.
%\vspace{-1.5em}\paragraph{Cloud Profilers:}~\cite{interference-profiling-in-cloud} describes a profiling system that measures the interdependence between application performance and CPU steal time due to co-tenant interference in cloud applications. Systems such as this help build the case that if tenant's contention for shared resources such as CPU and memory can be reduced, applications can achieve better performance in a  multi-tenant cloud environment.
\vspace{-1.5em}\paragraph{Satisfying SLAs:} Work on distributed systems storage has looked at satisfying latency and consistency SLOs. For example, Pileus~\cite{terry2013consistency} is a storage system that allows users to specify multi-level SLA requirements. During favorable conditions, the system can deliver responses with ideal consistency and latency. When conditions deteriorate, it refers to the user's SLA specification to decide whether to prefer consistency or low latency when fetching results. Tuba~\cite{ardekani2014self} builds on the functionality of Pileus and performs reconfiguration to adapt to changing workloads to meet performance requirements. 
SPANStore~\cite{wu2013spanstore} is a geo-replicated storage service that trades off cost and latency, while satisfying consistency and fault-tolerance %SPANStore~\cite{wu2013spanstore} is a geo-replicated storage service that spans multiple cloud services and tries to automate the process of trading off cost and latency, while satisfying consistency and fault-tolerance requirements.

To the best of our knowledge, Henge is the first work that combines elastic resource management for stream processing systems in a multi-tenant environment.


\end{comment}

==> henge-arxiv 2/text/13-conclusion.tex <==
\vspace{-1.0em}
\section{Conclusion}
\label{conclusion}

We presented Henge, a system for intent-driven (SLO-based) multi-tenant stream processing. Henge provides SLO satisfaction for topologies (jobs) with  latency and/or throughput requirements. To make throughput SLOs independent of input rate and topology structure, Henge uses a new  relative throughput  metric called juice.  In a cluster, when jobs  miss their SLO, Henge uses three kinds of actions (reconfiguration, reversion or reduction) to improve the sum utility achieved by all jobs throughout the cluster. Our experiments with real Yahoo! topologies and Twitter datasets have shown that in multi-tenant settings with a mix of SLOs, Henge: 
i) converges quickly to max system utility when resources suffice; 
ii) converges quickly to a high system utility when the cluster is constrained; 
iii) gracefully handles dynamic workloads, both abrupt (spikes, natural fluctuations) and gradual (diurnal patterns, Twitter datasets);
iv) scales gracefully with cluster size and number of jobs; and
v) is failure tolerant. % requirements
%Our results show that it can provide 95-100\% SLO satisfaction on a multi-tenant cluster, reduces resource consumption by 40\% and scales linearly with increasing topologies on a cluster. 




%\ig{replace emph headings with bf. I've done most. Do any I missed.}

% \ig{please check all these percentiles and the description about them. the reviewer has to find only one of them incorrect to reject the paper.}

% \ig{Double check correctness of all figures. And consistency of their captions.}

% \ig{Double-Check all equations please for correctness.}

% \ig{please doublecheck all juice examples for correctness.}


% \ig{make sure our text is flush to the bottom of 12 pages (else reviewers will say that we did not do enough work - not kidding). }

% \ig{please please pretty please distinguish between terms max utility and utility, everywhere in the paper. utility term by itself refers to current utility. better not use unqualified utility term at all. this above term should be max utility. it is small things like this confuse and distract reviewers!}

% \ig{i'm finding 1000s, 900 seconds, and also 920 s, and so on, all in the text. please be consistent! These should be 1000 s, 900 s, 920 s, and so on. again, small things that distract reviewers from your main message.}


%\ig{Fig.~\ref{star-juice} caption is being covered by the figure below it. Please check the *pdf* not the sharelatex compile visible, since these are obviously inconsistent. }


%\ig{please increase the size of figures that are too small, now that we are under page limit again.}


% \ig{Your references need to be consistent in format and capitalize systems names (use curly braces).

% \squishlist
% \item Some of your references use capitals for intermediate words (18, 19) while others don't (22, 38, 24, 27, 30, 41, 46, 48, 52, 55, 56, ... there are many more). Check all references.

% \item References that are inconsistent in conference naming (they don't use the long form): 54, 57,  19, 68, 38,  (there are others).

% \item Some conferences use sixth while others use 6th. Make all consistent.

% % \item 78 (Stela) needs to be anonymized (replace with XXX).
% \item References that need to capitalize something: 26, 41, 44, 71, 72, 73, 77, (there are others).
% \\item References that are botched: 41 (conf name), 43 (no conf name), (there are others).  
% \squishend

% }

==> text/11c-henge-policy-eval-figs.tex <==
\begin{figure*}
	\centering
	\begin{minipage}{1\columnwidth}
		\centering
		\includegraphics[width=1\columnwidth]{figures/simple-convergence/exp72/figure14.pdf} % \
		\caption{Right top: Topologies are chosen for reconfiguration based on which has worst performance. Right bottom: The improvement in total utility due to reconfiguration. Left: $99^{th}$ percentile latency improves due to reconfigurations. \fkc{Don't use moving average for tail latency}	}	\label{equal}
	\end{minipage}\hfill
	\begin{minipage}{1\columnwidth}
		\centering
		\includegraphics[width=1\columnwidth]{figures/simple-convergence/exp109/figure15.pdf} % second figure itself
		\caption{Topologies are chosen for reconfiguration, first in order of priority, and second in order of poor performance. Therefore, the T1-T3 are chosen first (utility=35), and T4 (utility=5) is chosen last. Right bottom: reconfiguring T1-T3 provides most increase in overall utility. \fkc{Make points bigger}
		}
	
				\label{unequal}
	\end{minipage}
\end{figure*}

\begin{figure}[t]
	\vspace{-0.7cm}
	\centering
	\includegraphics[width=0.8\columnwidth]{figures/reversion.pdf}
			\vspace{-0.2cm}
		% This is exp 134
	\caption{A cluster of 10 topologies (utility of each topology=5) converges after reversion}
	\label{reversion-reduction}
\end{figure}

\begin{figure}[h!]
	\vspace{-0.5cm}	
	\begin{center}
				\includegraphics[width=1.0\columnwidth]{figures/hybrid/hybrid.pdf}
			\caption{Hybrid SLOs: the first and second reconfiguration help meet the juice and latency SLO respectively }
			
		\label{hybrid}
	\end{center}
\vspace{-0.2cm}
\end{figure}



\begin{figure}[t]
	\vspace{-0.3cm}	
		\begin{center}
			\includegraphics[width=1.0\columnwidth]{figures/fairness/all.pdf}
    \caption{Topologies are no longer reconfigured (during time indicated in dotted green) as they do not show more than 5\% improvement in last reconfiguration}
	\label{fairness}
			\end{center}
		\vspace{-0.6cm}	
\end{figure}
	


\begin{figure*}
	\centering
	\begin{minipage}{1\columnwidth}
				\vspace{-0.6cm}
		\centering
		\includegraphics[width=1\columnwidth]{figures/simple-convergence/exp95/figure19.pdf} % first figure itself

		\vspace{-0.3cm}
		\caption{Reconfiguration allows a topology to adjust to a spike in input rate}
		\label{spike}
		\vspace{-0.5cm}
	\end{minipage}\hfill
	\begin{minipage}{1\columnwidth}
				\vspace{-0.5cm}
		\centering
		\includegraphics[width=1\columnwidth]{figures/diurnal/diurnal_2.pdf} % second figure itself
		\caption{Diurnals are a common pattern in internet traffic. Henge reconfigures a topology so it is able to meet its SLO of 60 ms during peak loads.}
		\label{diurnal}
				\vspace{-0.1cm}
	\end{minipage}

\end{figure*}

